Transport map accelerated Markov chain Monte Carlo

We introduce a new framework for efficient sampling from complex probability distributions, using a combination of optimal transport maps and the Metropolis-Hastings rule. The core idea is to use continuous transportation to transform typical Metropolis proposal mechanisms (e.g., random walks, Langevin methods) into non-Gaussian proposal distributions that can more effectively explore the target density. Our approach adaptively constructs a lower triangular transport map-an approximation of the Knothe-Rosenblatt rearrangement-using information from previous MCMC states, via the solution of an optimization problem. This optimization problem is convex regardless of the form of the target distribution. It is solved efficiently using a Newton method that requires no gradient information from the target probability distribution; the target distribution is instead represented via samples. Sequential updates enable efficient and parallelizable adaptation of the map even for large numbers of samples. We show that this approach uses inexact or truncated maps to produce an adaptive MCMC algorithm that is ergodic for the exact target distribution. Numerical demonstrations on a range of parameter inference problems show order-of-magnitude speedups over standard MCMC techniques, measured by the number of effectively independent samples produced per target density evaluation and per unit of wallclock time.

==> Paper4Arxiv 2/ESS_Calculation.tex <==
\section{ESS Calculation Details}\label{sec:esscalc}
Here we describe the calculation of the maximum integrated autocorrelation time $\tau_{\text{max}}$ used throughout our results.  Assume we are given $M$ independent MCMC chains on an $n$-dimensional parameter space.   Then, let $\tau_{i,j}$ be the integrated autocorrelation time of dimension $j$ on chain $i$.  This value is computed by applying the Fourier transform method from \cite{Wolff2004} to each dimension of each chain independently.  We then define $\tau_{\text{max}}$ as 
\begin{equation}
\tau_{\text{max}} = \max_{j\in\{1,\ldots,n\}} \left[ \underset{i\in\{1,\ldots, M\}}{\text{median}}\left( \tau_{i,j} \right) \right],
\end{equation}
where the median is taken over the chains and the maximum (worst case) is taken over dimensions.  

Effective sample size (ESS) is calculated similarly.  Let $\text{ESS}_{i,j} = \frac{K}{2\tau_{i,j}}$, where $K$ is the number of post-burn-in samples in each chain.  The reported ESS is then given by 
\begin{equation}
\text{ESS} = \min_{j\in\{1,\ldots, n\}} \left[ \underset{i\in\{1,\ldots, M\}}{\text{median}} \left( \frac{K}{2\tau_{i,j}}\right) \right].
\end{equation}
Note that while ESS uses only the samples produced after the burn-in period, normalized values of ESS reported in Section \ref{sec:perf} (e.g., ESS per function evaluation and ESS per second of wallclock time) use \emph{all} function evaluations or computational time in evaluating the denominator. Thus the cost of burn-in is reflected in these normalized performance metrics.

==> Paper4Arxiv 2/MCMC_Convergence.tex <==
%\subsection{Setting the stage: some definitions and fundamental theorems}
%\begin{definition}[Exponentially light density]
%Let $\td(\trv)$ be a probability density.  Now consider the quantity
% \begin{equation}
% \limsup_{\|\trv\|\rightarrow \infty} \frac{\trv}{\|\trv\|}\cdot \nabla \log \td(\trv) \label{eq:expLight}
% \end{equation}
% We call $\td(\trv)$:
% \begin{itemize}
% \item super-exponentially light when (\ref{eq:expLight}) is $-\infty$
% \item exponentially light when (\ref{eq:expLight}) is negative
% \item sub-exponentially light when (\ref{eq:expLight}) is $0$
% \end{itemize}
%\rule{\textwidth}{0.4pt}\\*%
%\end{definition}




%\begin{theorem}[Geometric ergodicity of random walk]
%\label{thm:rmGeo}
%Let $q(\trv^\prime | \trv) = N(\trv,\sigma_q^2I)$ be a symmetric random walk proposal density with variance $\sigma_q^2$.  From theorem 4.3 of \cite{Jarner2000}, the Metropolis-Hastings rule produces a geometrically ergodic MCMC chain for a target density $\td(\trv)$ when the following conditions hold
%\begin{enumerate}
%\item The target density is super-exponentially light (i.e. (\ref{eq:expLight}) is $-\infty$
%\item The curvature condition holds:
%\begin{equation}
% \limsup_{\|\trv\|\rightarrow \infty} \frac{\trv}{\|\trv\|}\cdot \frac{\nabla \log \td(\trv)}{\|\nabla \log \td(\trv)\|} < 0 \label{eq:curvature}
%\end{equation}
%\end{enumerate}
%\end{theorem}
%\begin{proof}
%See theorem 4.3 of \cite{Jarner2000}.
%\end{proof}
%\noindent\rule{\textwidth}{0.4pt}\\*%
%
%\subsection{Geometric ergodicity of fixed map MCMC}
%Assume I have a fixed transport map $T(\trv)=\rrv$.  This section will show that under some bounded derivative assumptions and super-exponentially light target distribution $\td(\trv)$, the map-based MCMC algorithm is geometrically ergodic.  This is summarized in the following theorem.
%
%\begin{theorem}[Geometric ergodicity of fixed map MCMC]
%\label{thm:mapGeo}
%Let $\td(\trv)$ be a super-exponentially light density, and let $q_\rrv(\rrv^\prime | \rrv)$ be a reference proposal $\rrv$ that yields a geometrically-ergodic MCMC chain for super-exponentially light densities.  Now, assume that we have a lower triangular map $\imap(\trv)$ and scalars $0<d_{min} < d_{max}<\infty$ such that 
%\begin{equation}
%\max_{i,j\in\{1,2,...,\pd\}} \sup_{\trv\in\real^\pd} \frac{\partial \imap_i(\trv)}{\partial \trv_j} \leq d_{max} \label{eq:dUB}
%\end{equation}
%and
%\begin{equation}
%\min_{i,j\in\{1,2,...,\pd\}} \inf_{\trv\in\real^\pd} \frac{\partial \imap_i(\trv)}{\partial \trv_j} \geq d_{min}\label{eq:dLB}
%\end{equation}
%For such a map, the fixed-map MCMC algorithm is geometrically ergodic.\\
%\end{theorem}
%\noindent\rule{\textwidth}{0.4pt}\\*%

%\begin{proof}
%For any monotone map $\imap(\trv)$, the inverse map yields a density on the $\rrv$-space.  This density, call it $\td_\rrv(\rrv)$ is given by:
%\[
%\td_\rrv(\rrv) = \td(\imap^{-1}(\rrv))|\mbox{det}D_\rrv \imap^{-1}(\rrv)|
%\]
%So, 
%\begin{equation}
%\frac{\rrv}{\|\rrv\|}\cdot \nabla \log \td_\rrv(\rrv) = \frac{\rrv}{\|\rrv\|}\cdot \left(\nabla\log\td(\imap^{-1}(\rrv)) + \sum_{i=1}^\pd \nabla \log\frac{\partial \imap^{-1}_i(\rrv)}{\partial \rrv_i}\right)
% \end{equation}
% 
%\begin{eqnarray}
%\frac{\rrv}{\|\rrv\|}\cdot \nabla \log \td_\rrv(\rrv) &=& \frac{\rrv}{\|\rrv\|}\cdot \nabla\log\td(\imap^{-1}(\rrv)) + \frac{1}{\|\rrv\|}\sum_{i=1}^\pd r_i\left(\frac{\partial \imap^{-1}_i(\rrv)}{\partial \rrv_i}\right)^{-1} \frac{\partial^2 \imap^{-1}_i(\rrv)}{\partial \rrv_i^2} \nonumber\\ 
%&\leq&  \frac{\rrv}{\|\rrv\|}\cdot \nabla\log\td(\imap^{-1}(\rrv)) + \frac{1}{\|\rrv\|}\sum_{i=1}^\pd r_i d_{max}d_{2max} \nonumber \\ 
%&=&  \frac{\rrv}{\|\rrv\|}\cdot \nabla\log\td(\imap^{-1}(\rrv)) + C_1 \label{eq:bound1}\\ 
% \end{eqnarray}
%Notice that the  $\frac{\rrv}{\|\rrv\|}\cdot \nabla\log\td(\imap^{-1}(\rrv))$ term in this expression is simply a directional derivative.  We are taking the derivative of $\log\td(\imap^{-1}(\rrv))$ in the $\frac{\rrv}{\|\rrv\|}$ direction.  Let $C\cap\real^\pd$ be the space of $\pd$ dimensional unit vectors.  We know:
%\begin{equation}
%\lim_{t\rightarrow \infty} \sup_{d\in C}\frac{\partial}{\partial t} \log\td\left(t d\right) = -\infty \label{eq:bound2}
%\end{equation}
%and we would like to characterize the following expression:
%\[
%\lim_{t\rightarrow \infty} \sup_{d\in C} \frac{\partial}{\partial t} \log\td\left(\imap^{-1}\left(td\right)\right)
%\]
%\[
%\lim_{t\rightarrow \infty} \sup_{d\in C} \frac{\partial}{\partial t} \log\td\left(\|\imap^{-1}\left(td\right)\| \frac{\imap^{-1}\left(td\right)}{\|\imap^{-1}\left(td\right)\|}\right)
%\]
%\[
%\lim_{t\rightarrow \infty} \sup_{d\in C} \frac{\partial}{\partial t} \log\td\left(\|\imap^{-1}\left(td\right)\| \frac{\imap^{-1}\left(td\right)}{\|\imap^{-1}\left(td\right)\|}\right) = \lim_{t_2\rightarrow \infty} \sup_{d\in C} \frac{\partial}{\partial t_2}\left[ \log\td\left(t_2 \frac{\imap^{-1}\left(td\right)}{\|\imap^{-1}\left(td\right)\|}\right)\right]\frac{\partial t_2}{\partial t}
%\]
%Now, because the derivatives of $\imap^{-1}$ are bounded below by $1/d_{max}$ and above by $1/d_{min}$, the $\partial t_2/\partial t$ term is bounded.  Moreover, because of (\ref{eq:bound2}), this means that 
%\begin{equation}
%\lim_{t\rightarrow \infty} \sup_{d\in C}\frac{\partial}{\partial t} \log\td\left(\imap^{-1}(t d)\right) = -\infty \label{eq:bound3}
%\end{equation}
%Now, combining this with (\ref{eq:bound1}), gives me 
%\[
%\lim_{\|\rrv\|\rightarrow \infty} \frac{\rrv}{\|\rrv\|}\cdot \nabla \log \td_\rrv(\rrv) = -\infty
%\]
%This means that $\td_\rrv(\rrv)$ is super-exponentially light.  However, for the random walk to converge geometrically, we also need to satisfy the curvature condition from (\ref{eq:curvature}).  {\color{red} I believe the monotonicity of our map will give us this automatically.}
%
%
%\end{proof}
%\noindent\rule{\textwidth}{0.4pt}\\*%
%
%Let $R$ be a large scalar, assume that our map is defined by:
%\begin{equation}
%\imap(\trv) = \left\{ \begin{array}{ll} P(\trv) & \quad \|\trv\|\leq R\\ P\left(R\frac{\trv}{\|\trv\|}\right) + \left(\frac{\trv}{\|\trv\|}\cdot \nabla P\left(R\frac{\trv}{\|\trv\|}\right)\right)(\|\trv\|-R)\frac{\trv}{\|\trv\|} &  \quad \|\trv\|> R \end{array}\right.
%\end{equation}
%where $P$ is some strictly monotone polynomial map.  A map $\imap(\trv)$ defined by this expression satisfies the derivative constraints we need to prove convergence.  Note that in practice, $R$ can be chosen quite large and is not incorporated into the code.
%
\section{Proof of ergodicity}\label{sec:detailedConvergence}
Section \ref{sec:convergence} of the paper provides an overview of the
convergence properties of our map-accelerated MCMC algorithm.  In this
appendix, we include some of the associated technical analysis.  In
particular, we provide detailed proofs of Lemma~\ref{lem:propBnds} and
Lemma~\ref{lem:dimAdapt}. The remaining results needed for Theorem \ref{thm:ergodic} are direct extensions of the proof of Lemma 6.1 in \cite{Atchade2006}.

\subsection{Bounded target proposal}
The goal of this section is to prove Lemma \ref{lem:propBnds} by finding two zero-mean Gaussian densities that bound the map-induced target-space proposal density $q_{\trv,\bar{\mapp}}$.  We assume throughout this appendix that the target density $\pi(\trv)$ is finite, continuous, and super-exponentially light. (See \eqref{eq:superLight} for the definition of super-exponentially light.)  We also assume that the reference proposal density $q_\rrv(\rrv^\prime | r)$ is a Gaussian random walk with a location-dependent bounded drift term $m(\rrv)$ and fixed covariance $\Sigma$.  Such a proposal takes the form
\begin{equation}
q_\rrv(\rrv^\prime | r) = N(\rrv+m(\rrv), \Sigma).
\end{equation}
Given this proposal density, we can follow \cite{Atchade2006} and show that there exist two zero-mean Gaussian densities $g_1$ and $g_2$, as well as two scalars $k_1$ and $k_2$, such that $0<k_1<k_2<\infty$ and 
\begin{equation}
k_1 g_1(\rrv^\prime - \rrv) \leq q_\rrv(\rrv^\prime | \rrv) \leq k_2 g_2(\rrv^\prime - \rrv)\label{eq:propBounds}.
\end{equation}
Now, we will use the bi-Lipschitz condition in \eqref{eq:dUB} to bound the target space proposal $q_{\trv,\bar{\mapp}}$ as required by Lemma \ref{lem:propBnds}.

\begin{proof}[Proof of Lemma \ref{lem:propBnds}]
%\paragraph{Proof of Lemma 1.}
The following s.pdf yield an upper bound:
\begin{eqnarray}
q_{\trv,\bar{\mapp}}(\trv^\prime \vert \trv ) & = & q_\rrv(\imap(\trv^\prime) \vert \imap(\trv)) |\det \dimap(\trv^\prime)|\label{eq:tqUB1}  \nonumber \\
& \leq & q_\rrv(\imap(\trv^\prime) \vert \imap(\trv))  \lambda_{\text{max}}^\pd\label{eq:tqUB2}  \nonumber \\
& \leq & k_2g_2(\imap(\trv^\prime) - \imap(\trv)) \lambda_{\text{max}}^\pd\label{eq:tqUB3}  \nonumber \\
& \leq & \left(k_2 \lambda_{\text{max}}^\pd\right)g_2\left( \lambda_{\text{min}}\left(\trv^\prime-\trv\right)\right)\label{eq:tqUB4} \nonumber \\
& = & k_{U}g_U\left(\trv^\prime-\trv\right)\label{eq:tqUB},
\end{eqnarray}
where $g_U$ is another zero-mean Gaussian.  Moving from the second line to the third line above is a consequence of \eqref{eq:dUB}. Moving from the third line to the fourth line uses the lower bound in \eqref{eq:dUB} and the fact that $g_2$ is a Gaussian with zero mean, which implies that $g_2(x_1)>g_2(x_2)$ when $\|x_1\|<\|x_2\|$.  Notice that $k_U$ does not depend on the particular coefficients of the map $\imap$; it only depends on the Lipschitz constant in \eqref{eq:dUB}. A similar process can be used to obtain the following lower bound:
\begin{eqnarray}
q_{\trv,\bar{\mapp}}(\trv^\prime \vert \trv ) & = & q_\rrv(\imap(\trv^\prime) \vert \imap(\trv)) |\det\dimap(\trv^\prime)|\nonumber \\
& \geq & q_\rrv(\imap(\trv^\prime) \vert \imap(\trv))  \lambda_{\text{min}}^\pd \nonumber \\
& \geq & k_1g_1(\imap(\trv^\prime) - \imap(\trv)) \lambda_{\text{min}}^\pd \nonumber \\
& \geq & \left(k_1 \lambda_{\text{min}}^\pd \right)g_1\left( \lambda_{\text{max}}\left(\trv^\prime-\trv\right)\right)\nonumber \\
& = & k_{L}g_L\left(\trv^\prime-\trv\right)\label{eq:tqLB}.
\end{eqnarray}
Lemma \ref{lem:propBnds} follows directly from (\ref{eq:tqUB}) and (\ref{eq:tqLB}).
\end{proof}

\subsection{SSAGE}

With (\ref{eq:tqUB}) and (\ref{eq:tqLB}) in hand, the proof of Lemma 6.1 in  \cite{Atchade2006} yields Lemma \ref{lem:minor}: the minorization component of the SSAGE condition.  Thus, to show SSAGE, we only need to establish Lemma \ref{lem:drift}.  Our proof of Lemma \ref{lem:drift} is built on the intermediate Lemmas \ref{lem:part1} and \ref{lem:part2} provided below and on the proof of Lemma 6.2 in \cite{Atchade2006}.

For the arguments below, we will use the Metropolis-Hastings transition kernel given by
 \begin{equation*}
P_{\bar{\mapp}}(x,dy) = \alpha_{\bar{\mapp}}(x,y)q_{\trv,{\bar{\mapp}}}(y\vert x)dy + r_{\bar{\mapp}}(x)\delta_x(dy),
\end{equation*}
where
 \begin{equation*}
r_{\bar{\mapp}}(x) = 1-\int \alpha_{\bar{\mapp}}(x,y)q_{\trv,{\bar{\mapp}}}(y\vert x)dy,
\end{equation*}
and $\alpha$ is the Metropolis-Hastings acceptance probability given by
 \begin{equation*}
\alpha_{\bar{\mapp}}(x,y) = \min\left\{1, \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x \vert  y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y \vert x)}
\right\} .
\end{equation*}
We will also use the set of guaranteed acceptance, given by
\begin{equation*}
A_{\bar{\mapp}}(x) = \left\{ y\in \real^\pd : \pi(y)q_{\theta,{\bar{\mapp}}}(x\vert y)\geq \pi(x)q_{\theta,{\bar{\mapp}}}(y\vert x)\right\},
\end{equation*}
and the set of possible rejection, simply defined as the complement of the set above:
\begin{equation*}
R_{\bar{\mapp}}(x) = A_{\bar{\mapp}}(x)^C .
\end{equation*}

 \begin{lemma}\label{lem:part1}
Let $V(x) = c_V\td^{-\alpha}(x)$ be a drift function defined by some $\alpha\in (0,1)$.  The constant $c_V= \sup_{x} \pi^\alpha(x)$ is chosen so that $\inf_x V(x) = 1$.  Then the following holds:
\begin{equation}
\limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \, \frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} < \limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \,  \int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy \label{eq:part1Goal}.
\end{equation}
 \end{lemma}
\begin{proof}%[Proof of Lemma \ref{lem:part1}]
First, we decompose the left-hand side of (\ref{eq:part1Goal}) into
\begin{eqnarray}
\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} &=& \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy + \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy \nonumber\\
&&+ \int_{R_{\bar{\mapp}}(x)} \left(1-\frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)} \right) q_{\trv,{\bar{\mapp}}}(y |x) dy \label{eq:part1Portions}.
\end{eqnarray}
Following the proof of Lemma 6.2 in \cite{Atchade2006}, we can show that the first two integrals in (\ref{eq:part1Portions}) go to zero as $\|x\|\rightarrow \infty$.  With that, we have
\begin{eqnarray}
\limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \, \frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}  &=& \limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \, \int_{R_{\bar{\mapp}}(x)} \left(1-\frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)} \right) q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber \\
&<& \limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \, \int_{R_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy.
\end{eqnarray}
The inequality results from the fact that  $[\td(y) q_{\trv,{\bar{\mapp}}}(x | y)]/[\td(x) q_{\trv,{\bar{\mapp}}}(y |x)]<1$ when $y \in R_{\bar{\mapp}}(x)$.
\end{proof}
\smallskip

\begin{lemma}\label{lem:part2}
The proposal has a nonzero probability of acceptance, i.e.,
 \begin{equation}
\int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy < 1. \label{eq:part2Goal}
\end{equation}
 \end{lemma}
\begin{proof}%[Proof of Lemma \ref{lem:part2}]
A nonzero probability of acceptance occurs if and only if there is a measurable set $W(x)\subset A_{\bar{\mapp}}(x)$.  To show that $W(x)$ exists, consider a small ball of radius $R$ around $x$.  Since $g_L$ and $g_U$ are zero mean and have positive variance, this implies
\begin{equation}
\inf_{y\in B(x,R)} \inf_{\bar{\mapp}} \frac{q_{\trv,{\bar{\mapp}}}(x|y)}{q_{\trv,{\bar{\mapp}}}(y|x)}  \geq  \inf_{y\in B(x,R)} \frac{k_Lg_L(x-y)}{k_Ug_U(y-x)} \geq  c_0 \, ,
\end{equation}
for some $c_0>0$.  Because $\td(x)$ is super-exponentially light, for any $u\in(0,R)$, there exists a radius $r_4$ such that $\| x \| > r_4$ implies
\[
\td\left(x-u\frac{x}{\|x\|}\right) \geq \frac{\td(x)}{c_0}.
\]
Subsequently, for any map coefficients, the acceptance probability for $x_1 = x-u\frac{x}{\|x\|}$ is one, which implies that $x_1\in A_{\bar{\mapp}}(x)$.  Now, define $W(x)$ as
\[
W(x) = \left\{ x_1-a\zeta, \, 0<a<R-u, \, \zeta \in S^{\pd-1},\, \left\|\zeta - \frac{x_1}{\|x_1\|}\right\|<\frac{.pdfilon}{2}\right\},
\]
where $.pdfilon$ is an arbitrarily small scalar and $S^{\pd-1}$ is the unit sphere in $\real^\pd$ dimensions.  
%Without the $\left\|\zeta - \frac{x_1}{\|x_1\|}\right\|<\frac{.pdfilon}{2}$ restriction, $W(x)$ would simply be $B(x_1,R-u)\setminus \{x_1\}$.  
Note that $\left\|\zeta - x_1 / \|x_1\| \right\|<\frac{.pdfilon}{2}$ ensures that $W(x)$ is a cone of points closer to the origin than $x_1$.
Now, using the final paragraph of the proof of Lemma 6.2 in \cite{Atchade2006}, the curvature condition from \eqref{eq:curveCond} ensures that the target density is larger in $W(x)$ than at $x_1$.  Since $x_1$ was accepted, this means that everything in $W(x)$ will also be accepted and that $W(x)\subseteq A_{\bar{\mapp}}(x)$.  Subsequently, we obtain
\begin{eqnarray}
\lim_{\|x\|\rightarrow \infty}\int_{R_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy  &=& \lim_{\|x\|\rightarrow \infty} \left(1 - \int_{A_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\right)\nonumber\\
& \leq &  \lim_{\|x\|\rightarrow \infty}\left(1 -  \int_{W(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\right) \nonumber\\
& < &  1 \label{eq:finalOneDrift2},
\end{eqnarray}
where we have used the fact that $W(x)$ is a measurable subset of $A_{\bar{\mapp}}(x)$ for large $x$.
\end{proof}
\smallskip


With Lemmas \ref{lem:part1} and \ref{lem:part2} in hand, we can now proceed to the proof of Lemma \ref{lem:drift} (the drift condition) from the main text.

\begin{proof}[Proof of Lemma \ref{lem:drift}]
%\paragraph{Proof of Lemma 4.}
%From the proof of Lemma 6.2 in \cite{Atchade2006} and \cite{Jarner2000}, the following two conditions are equivalent to Lemma \ref{lem:drift}:
%\begin{equation}
%\sup_x\sup_{\bar{\mapp}}\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} <\infty,
%\label{eq:driftFinite}
%\end{equation}
%and
%\begin{equation}
%\limsup_{\|x\|\rightarrow\infty} \sup_{\bar{\mapp}}\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} < 1.
%\label{eq:oneDrift}
%\end{equation}
%To show these conditions are satisfied, we will develop a bound on $\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}$ that ensures (\ref{eq:driftFinite}) is satisfied.  
%
Recall our choice of drift function: $V(x) = c_V\td^{-\alpha}(x)$ for $\alpha\in (0,1)$.  Using this function and the definitions of $ P_{\bar{\mapp}}$, $R_{\bar{\mapp}}$, and $A_{\bar{\mapp}}$ we can show that
\begin{eqnarray}
\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} &=& \frac{\int_{\real^\pd} \td^{-\alpha}(y) P_{\bar{\mapp}}(x,dy)}{\td^{-\alpha}(x)} \label{eq:simple1} \nonumber \\
%& = & \int_{\real^\pd}\frac{ \td^{-\alpha}(y)}{\td^{-\alpha}(x)}  P_{\bar{\mapp}}(x,dy)\nonumber\\
%& = & \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy + \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
&& + \int_{R_{\bar{\mapp}}(x)} \left(1-\frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)} \right) q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
& = & \int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
&&+ \int_{R_{\bar{\mapp}}(x)}  \left(\frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} -1\right)\frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
%&\leq & Q_{\trv,{\bar{\mapp}}}(\trv,R_{\bar{\mapp}}(x))  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
&&+ \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
&\leq & 1  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \\
&& + \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy . \nonumber 
\end{eqnarray}
%
Within the region of possible rejection $R_{\bar{\mapp}}(x)$, the acceptance rates are all in $[0,1)$, which allows us to further simplify \eqref{eq:simple1} to obtain
\begin{eqnarray}
%\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}  &\leq& 1  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
%&&+ \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} &\leq& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
  &<& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  \int_{R_{\bar{\mapp}}(x)}  \frac{q_{\trv,{\bar{\mapp}}}^{-\alpha}(y |x)}{q_{\trv,{\bar{\mapp}}}^{-\alpha}(x|y)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
  &=& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  \int_{R_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}^{1-\alpha}(y |x)q_{\trv,{\bar{\mapp}}}^{\alpha}(x|y)dy\nonumber\\
  &\leq& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
  %&& +  \int_{R_{\bar{\mapp}}(x)} \left(k_Ug_U(y-x)\right)^{1-\alpha}\left(k_Ug_U(x-y)\right)^\alpha dy\label{eq:densBound1}\nonumber\\
  &\leq& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  k_U^2 \int_{R_{\bar{\mapp}}(x)} g_U(y-x)dy \nonumber\\
  &=& 1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy,
\end{eqnarray}
where we have used the density upper bound in (\ref{eq:tqUB}) and $C_R$ is a finite constant.  A similar application of (\ref{eq:tqUB}) over $A_{\bar{\mapp}}(x)$ yields
\begin{eqnarray}
%\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}  &\leq&1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} &\leq&1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{\alpha}(x)}{\td^{\alpha}(y)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
%&\leq& 1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{q_{\trv,{\bar{\mapp}}}^\alpha(x |y)}{q_{\trv,{\bar{\mapp}}}^\alpha(y |x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
&\leq& 1+C_R +\int_{A_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}^\alpha(x |y) q_{\trv,{\bar{\mapp}}}^{1-\alpha}(y |x)dy\nonumber\\
&\leq& 1+C_R +k_U^2\int_{A_{\bar{\mapp}}(x)} g_U(x-y)dy\nonumber\\
%&=& 1+C_R + C_A\nonumber\\
&<& \infty \label{eq:driftFiniteVerify}.
\end{eqnarray}
Using Lemma \ref{lem:part1} and Lemma \ref{lem:part2}, we also have that 
\begin{equation}
\limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \, \frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} < \limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \,  \int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy < 1.\label{eq:oneVerify}
\end{equation}
From the proof of Lemma 6.2 in \cite{Atchade2006}, which resembles the proofs in \cite{Jarner2000}, Lemma \ref{lem:drift} follows from simultaneously satisfying the bounds \eqref{eq:driftFiniteVerify} and \eqref{eq:oneVerify}.  
 \end{proof}



%The bounds given in (\ref{eq:tqUB}) and (\ref{eq:tqLB}) are a fundamental component of the convergence proofs below.  In fact, with these bounds in place, we can follow the proof of Lemma 6.2 in \cite{Atchade2006} almost exactly.

%\subsection{SSAGE}\label{sec:ssage}
%To show that our adaptive scheme is ergodic, we need to establish two conditions:
%\begin{enumerate}
%\item Diminishing adaptation
%\item Containment
%\end{enumerate}
%For Algorithm 1 of the main text, these conditions are established in Lemmas 2--4.  Below we provide proofs of these lemmas.  These proofs will use the set of guaranteed acceptance, which is given by
%\begin{equation}
%A_{\bar{\mapp}}(x) = \left\{ y\in \real^\pd : \pi(y)q_{\theta,{\bar{\mapp}}}(x|y)\geq \pi(x)q_{\theta,{\bar{\mapp}}}(y|x)\right\},
%\end{equation}
%and the set of possible rejection, simply defined by the complement
%\begin{equation}
%R_{\bar{\mapp}}(x) = A_{\bar{\mapp}}(x)^C .
%\end{equation}

\subsection{Diminishing adaptation}
%\begin{proof}[Proof of Lemma 2]
In addition to SSAGE and containment, Theorem \ref{thm:ergodic} requires diminishing adaptation (Definition \ref{def:dim}).  The following proof establishes the diminishing adaptation proposed in Lemma \ref{lem:dimAdapt}.
%\paragraph{Proof of Lemma 2.}
\begin{proof}[Proof of Lemma \ref{lem:dimAdapt}]
The proof of this lemma relies on continuity of the map with respect
to $\bar{\mapp}$ and the convergence of \eqref{eq:regopt} as the number
of samples $K\rightarrow \infty$.  Note that we do not require
\eqref{eq:regopt} (or \eqref{eq:mckl})) to converge to the minimizer of the true KL divergence.

When the MCMC chain is not at an adaptation step, $\bar{\mapp}^{(k+1)}=\bar{\mapp}^{(k)}$.  Thus, to show diminishing adaptation, we need to show that the difference between transition kernels at step $K$ and $K+K_U$ decreases as $K\rightarrow \infty$.  Mathematically, we require
\begin{equation}
\lim_{K\rightarrow \infty} \mathbb{P}\left(\sup_{x \in \real^\pd}\left\| \tk_{\bar{\mapp}^{(K)}}(x,\cdot) - \tk_{\bar{\mapp}^{(K+K_U)}}(x,\cdot)\right\|_{TV} \geq \delta_1\right) = 0
\label{eq:tvinprob} 
\end{equation}
for any $\delta_1>0$.  Because the maps are linear in $\bar{\mapp}$, for a fixed $x$, the mapping from $\bar{\mapp}$ to $\tk_{\bar{\mapp}}(x,A)$ is continuous for any $A$.  Combined with the fact that $q_{\trv,{\bar{\mapp}}}$ is bounded, we have that \eqref{eq:tvinprob} will be satisfied when  
 \begin{equation}
\lim_{K\rightarrow \infty}\mathbb{P}\left( \left\| \mapp_i^{(K+K_U)}  -\mapp_i^{(K)} \right\| \geq \delta\right) = 0, \label{eq:da_goal1}
\end{equation}
for any $\delta>0$ and all $i\in\{1,2,\ldots,\pd\}$ .  We now turn to proving \eqref{eq:da_goal1}.

Recall that $\bar{\mapp}^{(K)}$ is the minimizer of 
\eqref{eq:regopt}, which is based on a $K$-sample Monte Carlo approximation of the KL 
divergence.   To notationally simplify \eqref{eq:regopt}, we will now use the convention that $\log(0)=-\infty$ and define the objective functions $f_i^{(K)}(\mapp_i)$ and $f_i^{(K+K_U)}(\mapp_i)$
as
\begin{eqnarray}
f_i^{(K)}(\mapp_i) & = & \frac{1}{K}g(\mapp_i) +\frac{1}{K}\sum_{k=1}^{K}\left[  \frac12\imap^2_i(\trv^{(k)}; \mapp_i) - \log\left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}}\right] \label{eq:fkk}\\
f_i^{(K+K_U)}(\mapp_i) & = & \frac{1}{K}g(\mapp_i) + \frac{1}{K}\sum_{k=1}^{K+K_U}\left[  \frac12\imap^2_i(\trv^{(k)}; \mapp_i) - \log\left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}}\right].\label{eq:fkku}
\end{eqnarray}
From \eqref{eq:regopt}, it should be clear that 
\begin{eqnarray}
\mapp_i^{(K)} &=& \argmin f_i^{(K)}(\mapp_i)\\
\mapp_i^{(K+K_U)} &=& \argmin f_i^{(K+K_U)}(\mapp_i),
\end{eqnarray}
for all $i=\{1,2,...,\pd\}$.\footnote{Using the factor $\frac{1}{K}$
  in both \eqref{eq:fkk} and \eqref{eq:fkku} is intentional.
  Multiplying the objective in \eqref{eq:regopt} by any positive
  scalar will not affect the solution and the common value of $\frac{1}{K}$ used here simplifies the results later on.}
Combining these expressions, we have
\begin{equation}
f_i^{(K+K_U)}(\mapp_i) =  f_i^{(K)}(\mapp_i) + \frac{1}{K}\sum_{k=K+1}^{K+K_U}\left[  \frac12\imap^2_i(\trv^{(k)}; \mapp_i) - \log\left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}}\right].\label{eq:da_parts1}
\end{equation}
%Because the map is bi-Lipschitz \eqref{eq:dUB} and the proposal density is bounded by Gaussian densities (see Lemma \ref{lem:propBnds}), the sum in \eqref{eq:da_parts1} is finite with probability one.  
From Markov's inequality, we then have
\begin{equation}
\mathbb{P}\left[ \left| f_i^{(K+K_U)}(\mapp_i) -  f_i^{(K)}(\mapp_i) \right| \geq \delta_2 \right] \leq \frac{1}{K \delta_2}\mathbb{E}\left[\left| \sum_{k=K+1}^{K+K_U}\left(  \frac12\imap^2_i(\trv^{(k)}; \mapp_i) - \log\left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}}\right)\right| \right],\label{eq:func_markov}
\end{equation}
for any $\delta_2>0$ and all $\gamma_i$.  Notice that the expectation on the right hand side of this expression is finite because the map is bi-Lipschitz \eqref{eq:dUB}, the proposal density is bounded by Gaussian densities (see Lemma \ref{lem:propBnds}), and the map is linear for large $\|\theta\|$ (see \eqref{eq:ubMap}).  Thus, 
\begin{equation}
\lim_{K\rightarrow \infty} \mathbb{P}\left[ \left| f_i^{(K+K_U)}(\mapp_i) -  f_i^{(K)}(\mapp_i) \right| \geq \delta_2 \right]  = 0 \quad \forall \gamma_i. \label{eq:funcConv}
\end{equation}

We now show that this implies the convergence of $\| \mapp_i^{(K+K_U)}-\mapp_i^{(K)} \|$.  First, consider a set $\mathcal{C}^{(K)}$ that depends on $\delta_2$ and takes the form
\begin{equation}
\mathcal{C}^{(K)} = \left\{ \mapp_i \, : \, f_i^{(K)}(\mapp_i)-\delta_2 \leq f_i^{(K)}(\mapp_i^{(K)})+\delta_2 \right\} \label{eq:ck_conv}.
\end{equation}
By definition, $\mathcal{C}^{(K)}$ will always contain $\mapp_i^{(K)}$.    Recall that $f_i^{(K)}$ is convex and admits a unique global minimizer.  Thus, as $\delta_2\rightarrow 0$, the set $\mathcal{C}^{(K)}$ will collapse on $\mapp_i^{(K)}$ and the maximum distance between any two points in $\mathcal{C}^{(K)}$ will go to zero.  This implies that for any $\delta>0$, there exists a $\delta_2$ such that 
\begin{equation}
 \sup_{\mapp_i, \mapp_i^\prime \in \mathcal{C}^{(K)}} \|\mapp_i - \mapp_i^\prime\|  < \delta. \label{eq:ck_bounds}
\end{equation}
We will now combine this expression with \eqref{eq:funcConv}.  Notice that for any $\delta_2>0$, \eqref{eq:funcConv} implies that
\begin{equation}
\lim_{K\rightarrow \infty} \mathbb{P}\left( \mapp_i^{(K+K_U)} \in \mathcal{C}^{(K)} \right) = 1.
\end{equation}
Combining this result with \eqref{eq:ck_bounds} yields 
\begin{equation}
\lim_{K\rightarrow \infty} \mathbb{P}\left( \left\| \mapp_i^{(K+K_U)}
    -  \mapp_i^{(K)} \right\| \geq \delta \right) = 0 \, ,
\end{equation}
which is the desired condition in \eqref{eq:da_goal1}.
\end{proof}


% We now have all the components necessary for the proof of Theorem \ref{thm:ergodic} given in Section \ref{sec:convergence}.



%Establishing the minorization and simultaneous drift conditions needed for SSAGE, and subsequently for Theorem 1, is more difficult than proving diminishing adaptation.  The following sections tackles these two 
%conditions. Before proceeding, however, notice that the map $\imap(\trv;\bar{\mapp})$ induces a target space proposal 
%that is combined with the Metropolis-Hastings rule to obtain a transition kernel 
%denoted by $P_{\bar{\mapp}}(\trv,\cdot)$.  We will use ${\bar{\mapp}}$ as a subscript to indicate a dependence on a 
%particular choice of map.  In many cases our goal will be to construct results 
%that do not depend on ${\bar{\mapp}}$.
%
%For the following analysis, assume $\td(x)>0$ for all finite $x$ and let $V(x) = c_V\td^{-\alpha}(x)$ for $\alpha\in (0,1)$, where $c_V= \sup_{x} \pi^\alpha(x)$ is chosen so that $\inf_x V(x) = 1$.  Also, choose the set $C$ to be a ball with radius $R_C>0$, i.e., $C=B(0,R_C)$.  Clearly, because we assume $\td(x)>0$,  we immediately obtain $\sup_{x\in C} V(x)<\infty$.
% 
%\subsection{Minorization}
%
%In this section, we prove the minorization condition of Lemma 3 from the main text.  
%
%%\begin{proof}[Proof of Lemma 3]
%\paragraph{Proof of Lemma 3.}
%Our goal here is to find: (i) a scalar $\delta$ that does not depend on ${\bar{\mapp}}$ and (ii) a nontrivial measure $\nu_{\bar{\mapp}}(\cdot)$, such that the following minorization condition holds:
%\begin{equation}
%P_{\bar{\mapp}}(x,\cdot) \geq \delta \nu_{\bar{\mapp}}(\cdot).
%\end{equation}
%To define $\delta$, we refer to the form of the Metropolis-Hastings transition kernel given by
%\[
%P_{\bar{\mapp}}(x,dy) = \alpha_{\bar{\mapp}}(x,y)q_{\trv,{\bar{\mapp}}}(y|x)dy + r_{\bar{\mapp}}(x)\delta_x(dy),
%\]
%where 
%\[
%r_{\bar{\mapp}}(x) = 1-\int \alpha_{\bar{\mapp}}(x,y)q_{\trv,{\bar{\mapp}}}(y|x)dy,
%\]
%and $\alpha$ is the Metropolis-Hastings acceptance rate.  The acceptance rate is defined by
%\[
%\alpha_{\bar{\mapp}}(x,y) = \min\left\{1, \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}
%\right\} .
%\]
%Let $\tau$ be the minimum acceptance rate over all $x,y\in C$ and over all of the map-induced proposal densities.  In other words, $\tau$ is defined by
%\begin{equation}
%\tau = \inf_{\bar{\mapp}} \inf_{x,y \in C} \min\left\{1, \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}\right\} \label{eq:minxy}.
%\end{equation}
%Notice that lower bound in (\ref{eq:tqLB}) ensures we always have a positive acceptance rate $\tau>0$ because
%\[
%\td(y) q_{\trv,{\bar{\mapp}}}(x | y) \geq \td(y) k_{L}g_L(x-y)>0 \quad \forall x,y\in C.
%\]  
%Now, this minimum acceptance rate can be substituted back into the transition kernel to obtain
%\begin{eqnarray}
%P_{\bar{\mapp}}(x,dy) &=& \alpha_{\bar{\mapp}}(x,y)q_{\trv,{\bar{\mapp}}}(y|x)dy + r_{\bar{\mapp}}(x)\delta_x(dy) \nonumber\\
%&\geq& \tau q_{\trv,{\bar{\mapp}}}(y|x)dy + r(x) \delta_x(dy).
%\end{eqnarray}
%Again using our lower bound on $q_{\trv,{\bar{\mapp}}}(y|x)$ from (\ref{eq:tqLB}), we have
%\begin{eqnarray}
%P_{\bar{\mapp}}(x,dy) &\geq& \tau  k_{L}g_L(x-y) dy + r_{\bar{\mapp}}(x)\delta_x(dy) \nonumber\\
%&\geq& \tau  k_{L}g_L(x-y) dy\label{eq:transLower}.
%\end{eqnarray}
%Thus, for $x\in C$, we have a lower bound on $P_{\bar{\mapp}}(x,dy)$ that does not depend on the map parameters ${\bar{\mapp}}$.  Now, we need to remove the $x$-dependence of this bound.  Since $g_L$ is a Gaussian density, $\inf_{z\in C} g_L(z-y) >0$ and we can define a new density $g_{C}$ that is not dependent on $x$.  This density $g_{C}$ takes the form
%\[
%g_{C}(y) = \frac{\inf_{x\in C} g_L(x-y)}{\int_{y\in\real^\pd} \inf_{x\in C} g_L(x-y) dy}.
%\]
%Using this expression yields
%\begin{equation}
%P_{\bar{\mapp}}(x,dy) \geq  \tau  k_{C}g_{C}(y) dy\label{eq:transLower2},
%\end{equation}
%where $k_{C} = k_L \int_{y\in\real^\pd} \inf_{x\in C} g_L(x-y) dy$.   It may now be tempting to directly use the right hand side of this expression to define the minorization measure $\nu$.  However, this expression is only valid for $x\in C$ and $dy\subset C$, and we need the minorization measure to be defined for all measurable sets in $\real^\pd$.  Thus an alternative expression for $\nu$ is required.  \cite{Rosenthal2009} provides a nice example that can be adapted to this situation.  First, set $\delta = \tau k_{C}$ and define
%\begin{equation}
%\nu(A) = \frac{\int_{A \cap C} g_{C}(y) dy}{\int_{C} g_{C}(y) dy} .
%\end{equation}
%This expression defines a nontrivial measure and allows us to create a lower bound using (\ref{eq:transLower2}) but on sets outside of $C$.  Combining this expression with (\ref{eq:transLower2}), we obtain
%\begin{equation}
%P_{\bar{\mapp}}(x,A) \geq \delta \nu(A),
%\end{equation}
%which establishes the minorization condition.\qed
%%\end{proof}
%\smallskip
%
%The proof above gives us the minorization component of the SSAGE condition.  The next section shows that our algorithm also satisfies the drift condition.
%
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Drift condition}
%This section shows that our adaptive algorithm satisfies the drift condition from Lemma 4 of the main text.  Lemmas \ref{lem:part1} and \ref{lem:part2}, provided below, are needed in the proof.
%
% \begin{lemma}\label{lem:part1}
%Let $V(\cdot)$, $P_{\bar{\mapp}}(x,dy)$, $\bar{\mapp}$, and $R_{\bar{\mapp}}$ be defined as in Section \ref{sec:ssage}. Then we have
%\begin{equation}
%\limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \, \frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} < \limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \,  \int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy \label{eq:part1Goal}.
%\end{equation}
% \end{lemma}
%\begin{proof}%[Proof of Lemma \ref{lem:part1}]
%The integral on the left-hand side of (\ref{eq:part1Goal}) can be decomposed into an integral over $A_{\bar{\mapp}}(x)$ and an integral over $R_{\bar{\mapp}}(x)$ to obtain
%\begin{eqnarray}
%\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} &=& \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy + \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy \nonumber\\
%&&+ \int_{R_{\bar{\mapp}}(x)} \left(1-\frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)} \right) q_{\trv,{\bar{\mapp}}}(y |x) dy \label{eq:part1Portions}.
%\end{eqnarray}
%To show that this expression is less than the rejection rate $\int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy$ as $\|x\|\rightarrow \infty$, we will show that the first two integrals (\ref{eq:part1Portions}) go to zero as $\|x\|\rightarrow \infty$ and that the last integral is bounded by $\int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy$.  During this derivation, it will be useful to further decompose $A_{\bar{\mapp}}(x)$ and $R_{\bar{\mapp}}(x)$ into subsets.  This decomposition will be based on a ball of radius $R$ around $x$, $B(x,R)$, where $R$ implicitly depends on some tolerance $.pdfilon>0$ through the requirement that
%\begin{equation}
%\int_{B(x,R)} g_U(y-x) dy \geq 1-.pdfilon \label{eq:epsUpper}.
%\end{equation}
%In addition to this ball, the decomposition of $A_{\bar{\mapp}}(x)$ and $R_{\bar{\mapp}}(x)$ will also be based on the sets $C_{\td(x)}$ and $C_{\td(x)}(u)$ defined by
%\begin{equation}
%C_{\td(x)} = \{y \in \real^\pd : \, \td(y)=\td(x)\},
%\end{equation}
%and for $u>0$,
%\begin{equation}
%C_{\td(x)}(u) = \{ y+sn(y): \, y\in C_{\td(x)}, -u\leq s \leq u\},
%\end{equation}
%where $n(y) = y / \|y\|$.
%
%One can think of $C_{\td(x)}$ as a single contour of the target density and $C_{\td(x)}(u)$ as a narrow region surrounding that contour.  Now, we can define the following non-overlapping subsets of $A_{\bar{\mapp}}(x)$ and $R_{\bar{\mapp}}(x)$:
%\begin{eqnarray}
%A_1(x) &=& A_{\bar{\mapp}}(x) \cap B(x,R)^c \nonumber\\
%A_2(x) &=& A_{\bar{\mapp}}(x) \cap B(x,R) \cap C_{\td(x)}(u) \nonumber\\
%A_3(x) &=& A_{\bar{\mapp}}(x) \cap B(x,R) \cap C_{\td(x)}(u)^c\nonumber\\
%R_1(x) &=& R_{\bar{\mapp}}(x) \cap B(x,R)^c \nonumber\\
%R_2(x) &=& R_{\bar{\mapp}}(x) \cap B(x,R) \cap C_{\td(x)}(u) \nonumber\\
%R_3(x) &=& R_{\bar{\mapp}}(x) \cap B(x,R) \cap C_{\td(x)}(u)^c.
%\end{eqnarray}
%Note that $A_{\bar{\mapp}}(x) = A_1(x) \cup A_2(x) \cup A_3(x)$ and $R_{\bar{\mapp}}(x) = R_1(x) \cup R_2(x) \cup R_3(x)$.  Using this new subsets, reconsider the $A_{\bar{\mapp}}(x)$ component of (\ref{eq:part1Portions}).  We can rewrite the integral from (\ref{eq:part1Portions}) as
%\begin{eqnarray}
%\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy  & =  &\int_{A_1(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy + \int_{A_2(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\&& + \int_{A_3(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \label{eq:Aportions}.
%\end{eqnarray}
%Recall that we are trying to make sure that this integral goes to zero as $\|x\|\rightarrow\infty$, so that we can subsequently bound (\ref{eq:oneDrift}).  Thus, our intermediate goal is to show that each of the integrals in (\ref{eq:Aportions}) goes to zero as $\|x\|\rightarrow \infty$.  Recall the bound used in (\ref{eq:densBound1}), which is repeated here
%\[
%\frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x)\leq k_U^2g_U(x-y).
%\]
%Applying this bound to the first two integrals in (\ref{eq:Aportions}) yields
%\begin{eqnarray}
%\int_{A_1(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy &\leq&k_U^2\int_{A_1(x)} g_U(x-y) dy  \label{eq:A11}\nonumber\\
%\int_{A_2(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy &\leq&k_U^2\int_{A_2(x)} g_U(x-y) dy \label{eq:A21}.
%\end{eqnarray}
%A result from \cite{Jarner2000} will allow us to bound the right hand sides of (\ref{eq:A11}) and (\ref{eq:A21}) by first bounding the size of $A_1(x)$ and $A_2(x)$.
%
%In the proof of \cite[Theorem 4.1]{Jarner2000}, the authors show that for a large radius $r_1$  and $\|x\|\geq r_1$, the Lebesgue measure of $C_{\td(x)}(u)\cap B(x,R)$ is bounded by:
%\begin{equation}
%\lambda\left(C_{\td(x)}(u)\cap B(x,R)\right) \leq \frac{u}{R}\left(\frac{\|x\| + R}{\|x\| - R}\right)^{\pd-1}\lambda\left(C_{\td(x)}(u)\cap B(x,3R)\right)\label{eq:lebesgueBound}
%\end{equation}
%where $\pd$ is the dimension of $x$ and $\lambda$ is the Lebesgue measure. Notice that as $\|x\|\rightarrow \infty$, the right hand side of this expression becomes $u/R$.  Thus, by using the absolute continuity of the Gaussian density $g_U(y-x)$ with respect to Lebesgue measure, we can use the expression in (\ref{eq:lebesgueBound}) to find a width $u$ and a larger radius $r_2>r_1$ such that for any $.pdfilon > 0$
%\begin{equation}
%\int_{C_{\td(x)}(u)\cap B(x,R)} g_U(y-x)dy \leq .pdfilon \quad \mbox{ for } \|x\|\geq r_2\label{eq:epsLower}.
%\end{equation}
%By applying (\ref{eq.pdfLower}) to (\ref{eq:A21}) and (\ref{eq:epsUpper}) to (\ref{eq:A11}) we obtain the upper bounds
%\begin{eqnarray}
%\int_{A_1(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy &\leq&k_2^2.pdfilon  \label{eq:A12}\nonumber\\
%\int_{A_2(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy &\leq&k_2^2.pdfilon \label{eq:A22}.
%\end{eqnarray}
%Applying these expressions to (\ref{eq:Aportions}) shows that as $\|x\| \rightarrow \infty$, we can choose a contour width $u$ such that 
%\[
%\lim_{\|x\|\rightarrow \infty} \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy  = \lim_{\|x\|\rightarrow \infty}  \int_{A_3(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy .
%\]
%This takes care of the $A_1(x)$ and $A_2(x)$ portions of (\ref{eq:Aportions}).  However, we still need to show that the $A_3(x)$ portion goes to zero, i.e., $\lim\limits_{\|x\|\rightarrow \infty} \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy = 0$.  To show this, we will simply show that the size of the set $A_3(x)$ goes to zero as $\|x\|\rightarrow \infty$.  This will require the super-exponential characteristic of the target density $\pi(\trv)$.
%
%Continuing to follow the proof of Lemma 6.2 from \cite{Atchade2006}, for any $r>0$ and $a>0$, define 
%\[
%d_r(a) = \sup_{\|x\|\geq r} \frac{\td\left(x+a\frac{x}{\|x\|}\right)}{\td(x)}
%\]
%As \cite{Atchade2006} points out, $d_r(a)\rightarrow 0$ as $r\rightarrow \infty$ because the target density $\td(\trv)$ is super-exponentially light.  For a particular $r_3<\infty$, this convergence provides the following bound (taken from \cite{Atchade2006})
%\begin{equation}
% \int_{A_3(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) \leq d_{r_3}(\delta) \quad \mbox{ for all }\, \|x\| \geq r_3+R \label{eq:A32}.
%\end{equation}
%Now, combining (\ref{eq:A12}), (\ref{eq:A22}), and (\ref{eq:A32}), we can finally show
%\begin{equation}
%\lim_{\|x\|\rightarrow \infty} \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy = 0 \label{eq:Azero}.
%\end{equation}
%Moreover, the same reasoning that got us from (\ref{eq:Aportions}) to (\ref{eq:Azero}) can be used over the possible rejection region to show that
%\begin{equation}
%\lim_{\|x\|\rightarrow \infty} \int_{R_{\bar{\mapp}}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)} q_{\trv,{\bar{\mapp}}}(y |x) dy = 0. \label{eq:Rzero}
%\end{equation}
%With this simplification, the only remaining component on the right hand side of (\ref{eq:part1Portions}) is 
%\[
% \lim_{\|x\|\rightarrow \infty}\int_{R_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy.
%\]
%We therefore have (\ref{eq:part1Goal}). \qed
%\end{proof}
%\smallskip
%
%
% \begin{lemma}\label{lem:part2}
% Let the proposal $q_{\trv,{\bar{\mapp}}}$ and the set $R_{\bar{\mapp}}(x)$ be defined as before. Then the proposal has a nonzero probability of acceptance, i.e.,
%  \begin{equation}
%\int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy < 1. \label{eq:part2Goal}
%\end{equation}
% \end{lemma}
% \begin{proof}%[Proof of Lemma \ref{lem:part2}]
%We will show that there is a measurable set $W(x)\subset A_{\bar{\mapp}}(x)$.  Because $W(x)$ is in the guaranteed acceptance region, any $y$ proposed in $W(x)$ will be accepted with probability $1$.  Also notice that $W(x)$ does not depend on the map coefficients ${\bar{\mapp}}$.   
%
%For a small ball of radius $R$ around $x$, the following condition holds
%\begin{eqnarray}
%\inf_{y\in B(x,R)} \inf_{\bar{\mapp}} \frac{q_{\trv,{\bar{\mapp}}}(x|y)}{q_{\trv,{\bar{\mapp}}}(y|x)} & \geq & \inf_{y\in B(x,R)} \frac{k_Lg_L(x-y)}{k_Ug_U(y-x)}\label{eq:firstLineBound}\\
%& \geq & c_0, \nonumber
%\end{eqnarray}
%for some $c_0>0$.  The expression in (\ref{eq:firstLineBound}) is a result of $g_L$ and $g_U$ both having zero mean and positive variance.  Now, the fact that $\td(x)$ is super-exponentially light means that for $u\in(0,R)$, there is a radius $r_4$ such that when $\| x \| > r_4$, we have
%\[
%\td\left(x-u\frac{x}{\|x\|}\right) \geq \frac{\td(x)}{c_0}.
%\]
%This means that the acceptance probability for $x_1 = x-u\frac{x}{\|x\|}$ is one for any map coefficients ${\bar{\mapp}}$.  Mathematically, we have
%\[
%\frac{\td(x_1)}{\td(x)} \frac{q_{\trv,{\bar{\mapp}}}(x|x_1)}{q_{\trv,{\bar{\mapp}}}(x_1|x)}\geq \frac{\td(x_1)}{\td(x)} c_0 \geq 1.
%\]
%By our definition of the acceptance region $A_{\bar{\mapp}}(x)$, this means that $x_1\in A_{\bar{\mapp}}(x)$.  The single point $x_1$ has zero measure, requiring us to further show that there is a measurable set $W(x)$ around $x_1$.  Let $W(x)$ be defined as
%\[
%W(x) = \left\{ x_1-a\zeta, \, 0<a<R-u, \, \zeta \in S^{\pd-1},\, \left\|\zeta - \frac{x_1}{\|x_1\|}\right\|<\frac{.pdfilon}{2}\right\},
%\]
%where $.pdfilon$ is an arbitrarily small scalar and $S^{\pd-1}$ is the unit sphere in $\real^\pd$ dimensions.  Without the $\left\|\zeta - \frac{x_1}{\|x_1\|}\right\|<\frac{\epsilon}{2}$ restriction, $W(x)$ would simply be $B(x_1,R-u)\setminus \{x_1\}$.  However, this additional restriction forces the vector $\zeta$ to point in the same direction as $x$, which means that $W(x)$ is a cone of points closer to the origin than $x_1$.  Now, from the final paragraph of the proof of Lemma 6.2 in \cite{Atchade2006}, we know the curvature condition from (27*) ensures that the target density is larger in $W(x)$ than $x_1$.  Since $x_1$ was accepted, this means that everything in $W(x)$ will also be accepted and that $W(x)\subseteq A_{\bar{\mapp}}(x)$.  This implies that
%\begin{eqnarray}
%\lim_{\|x\|\rightarrow \infty}\int_{R_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy  &=& \lim_{\|x\|\rightarrow \infty} \left(1 - \int_{A_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\right)\nonumber\\
%& \leq &  \lim_{\|x\|\rightarrow \infty}\left(1 -  \int_{W(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\right) \nonumber\\
%& < &  1 \label{eq:finalOneDrift2},
%\end{eqnarray}
%where we have used the fact that $W(x)$ is a measurable subset of $A_{\bar{\mapp}}(x)$ for large $x$.  With (\ref{eq:finalOneDrift2}), we have proven (\ref{eq:part2Goal}).  \qed
%\end{proof}
%\smallskip
%
%
%
%With Lemmas \ref{lem:part1} and \ref{lem:part2} in hand, we can now proceed to the proof of Lemma 4 (Drift) from the main text.
%
%
%%\begin{proof}[Proof of Lemma 4]
%\paragraph{Proof of Lemma 4.}
%From the proof of Lemma 6.2 in \cite{Atchade2006}, which resembles the proofs in \cite{Jarner2000}, the following two conditions are equivalent to the SSAGE drift condition
%\begin{equation}
%\sup_x\sup_{\bar{\mapp}}\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} <\infty,
%\label{eq:driftFinite}
%\end{equation}
%and
%\begin{equation}
%\limsup_{\|x\|\rightarrow\infty} \sup_{\bar{\mapp}}\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} < 1.
%\label{eq:oneDrift}
%\end{equation}
%We will therefore satisfy the drift condition by satisfying both of these conditions.  First, we will develop a bound on $\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}$ that ensures (\ref{eq:driftFinite}) is satisfied.  
%
%Recall our choice of drift function: $V(x) = c_V\td^{-\alpha}(x)$ for $\alpha\in (0,1)$.  Plugging this function into (\ref{eq:driftFinite}) and simplifying yields
%\begin{eqnarray}
%\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} &=& \frac{\int_{\real^\pd} \td^{-\alpha}(y) P_{\bar{\mapp}}(x,dy)}{\td^{-\alpha}(x)} \label{eq:simple1}\\
%& = & \int_{\real^\pd}\frac{ \td^{-\alpha}(y)}{\td^{-\alpha}(x)}  P_{\bar{\mapp}}(x,dy)\nonumber\\
%& = & \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy + \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
%&& + \int_{R_{\bar{\mapp}}(x)} \left(1-\frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)} \right) q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
%& = & \int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
%&&+ \int_{R_{\bar{\mapp}}(x)}  \left(\frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} -1\right)\frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
%&\leq & Q_{\trv,{\bar{\mapp}}}(\trv,R_{\bar{\mapp}}(x))  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
%&&+ \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
%&\leq & 1  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
%&& + \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy . \label{eq:simple2}
%\end{eqnarray}
%%
%Within the region of possible rejection $R_{\bar{\mapp}}(x)$, the acceptance rates are all in $[0,1)$, which allows us to further bound (\ref{eq:simple1}) using (\ref{eq:simple2}) and the following algebra
%\begin{eqnarray}
%\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}  &\leq& 1  + \int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy \nonumber\\
%&&+ \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} \frac{\td(y) q_{\trv,{\bar{\mapp}}}(x | y)}{\td(x) q_{\trv,{\bar{\mapp}}}(y |x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
% &\leq& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  \int_{R_{\bar{\mapp}}(x)}  \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
%  &<& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  \int_{R_{\bar{\mapp}}(x)}  \frac{q_{\trv,{\bar{\mapp}}}^{-\alpha}(y |x)}{q_{\trv,{\bar{\mapp}}}^{-\alpha}(x|y)}q_{\trv,{\bar{\mapp}}}(y |x)dy\nonumber\\
%  &=& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  \int_{R_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}^{1-\alpha}(y |x)q_{\trv,{\bar{\mapp}}}^{\alpha}(x|y)dy\nonumber\\
%  &\leq& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
%  && +  \int_{R_{\bar{\mapp}}(x)} \left(k_Ug_U(y-x)\right)^{1-\alpha}\left(k_Ug_U(x-y)\right)^\alpha dy\label{eq:densBound1}\nonumber\\
%  &=& 1 +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy +  k_U^2 \int_{R_{\bar{\mapp}}(x)} g_U(y-x)dy \nonumber\\
%  &=& 1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy,
%\end{eqnarray}
%where the expression in (\ref{eq:densBound1}) is a consequence of the density upper bound in  (\ref{eq:tqUB}).  Now consider the region of guaranteed acceptance $A_{\bar{\mapp}}(x)$.  A similar application of (\ref{eq:tqUB}) over this region yields
%\begin{eqnarray}
%\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}  &\leq&1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{-\alpha}(y)}{\td^{-\alpha}(x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
%&=&1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{\td^{\alpha}(x)}{\td^{\alpha}(y)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
%&\leq& 1+C_R +\int_{A_{\bar{\mapp}}(x)} \frac{q_{\trv,{\bar{\mapp}}}^\alpha(x |y)}{q_{\trv,{\bar{\mapp}}}^\alpha(y |x)} q_{\trv,{\bar{\mapp}}}(y |x) dy\nonumber\\
%&=& 1+C_R +\int_{A_{\bar{\mapp}}(x)} q_{\trv,{\bar{\mapp}}}^\alpha(x |y) q_{\trv,{\bar{\mapp}}}^{1-\alpha}(y |x)dy\nonumber\\
%&\leq& 1+C_R +k_U^2\int_{A_{\bar{\mapp}}(x)} g_U(x-y)dy\nonumber\\
%&=& 1+C_R + C_A\nonumber\\
%&<& \infty \label{eq:driftFiniteVerify}.
%\end{eqnarray}
%Thus $\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)}$ is finite for all $x$ and ${\bar{\mapp}}$ and we have satisfied (\ref{eq:driftFinite}).  Furthermore, using Lemma \ref{lem:part1} and Lemma \ref{lem:part2}, we have that 
%\begin{equation}
%\limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \, \frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} < \limsup_{\|x\|\rightarrow \infty} \, \sup_{\bar{\mapp}} \,  \int_{R_{\bar{\mapp}}(x)}q_{\trv,{\bar{\mapp}}}(y |x) dy < 1.
%\end{equation}
%Thus, (\ref{eq:oneDrift}) is satisfied.  Using (\ref{eq:driftFinite}), (\ref{eq:oneDrift}), and the proof of Lemma 6.2 in \cite{Atchade2006}, our adaptive algorithm satisfies the SSAGE drift condition.\qed
%\smallskip
 
% \end{proof}
 



==> Paper4Arxiv 2/MapleModel.tex <==
\section{Maple exudation model details}\label{sec:maplemodel}
The forward model in Section \ref{sec:perf:maple} is a complicated system of differential-algebraic equations describing maple sap dynamics.  Here we give a minimal description of the model. Interested readers should consult the original derivation in \cite{Ceseri2013}. 

In addition to the differential algebraic system defined by \eqref{eq:MapleDae1}--\eqref{eq:MapleAlg5}, the volumes $V^v$ and $V_g^v(t)$ are given by
\begin{eqnarray*}
V^v &=& \pi (R^v)^2L^v\\
V_g^v(t) &=& \pi r(t)^2L^v\\
N&=& \frac{2\pi(R^f+R^v+W)}{2R^f+W}.
\end{eqnarray*}
The system is solved using MUQ~\cite{MUQ}, which in turn links to SUNDIALS~\cite{Sundials}.  The initial conditions for the state variables $s_{gi}$, $s_{iw}$, and $r(t)$ are derived from a steady state solution. We put $U(0)=0$.

The temperature field is assumed to be quasi-steady and is defined by the heat equation
\begin{align}
\partial_{x}\left(\kappa(x) \partial_x T(x,t)\right) & =  0 & \text{for } & x\in(\,s_{iw}(t),\, R^f+2R^v\,) \label{eq:Temperature} \\
T(x,t) & = 0 & \text{at } & x=s_{iw}(t) \nonumber \\ 
\kappa_w \partial_x  T(x,t)&= h(T_a(t)-T(x,t)) & \text{at } &
                                                              x=R^f+2R^v, \nonumber
\end{align}
where $T_a(t)$ is a transient temperature forcing at the edge of the computational domain ($x=R^f+2R^v$), $h=10$ is a heat transfer coefficient, and the thermal conductivity is defined piecewise as
\begin{equation*}
\kappa(x) = \left\{\begin{array}{cl}
 \kappa_w & x\in[\, s_{iw}(t),\, R_f+R_v-r(t)\,) \\
 \kappa_g & x\in[\, R_f+R_v-r(t),\, R_f+R_v+r(t)\,) \\
 \kappa_w & x\in[\, R_f+R_v+r(t),\, R_f+2R_v\,]\end{array}\right.  ,
\end{equation*}
where $\kappa_w$ is the thermal conductivity of water and  $\kappa_g$ is the thermal conductivity of air.  At any particular time, it is straightforward to solve \eqref{eq:Temperature} analytically, yielding a piecewise linear temperature field.

\begin{table}
\centering
\caption{Relationship between inference targets $\theta$ and model parameters for the maple problem.}
\begin{tabular}{|c|c|}\hline
Model variable & Transformation from $\theta$ \\\hline
$s_{gi}(0)$ & $(0.5\theta_2+ 0.5)\exp\left[0.2\log(\bar{R}^f)\theta_7 + \log(\bar{R}^f)\right]$\\
$s_{iw}(0)$ & $\exp\left[0.2\log(\bar{R}^f)\theta_7 + \log(\bar{R}^f)\right]$\\ 
$r(0)$ & $(0.5\theta_2+ 0.5)\exp\left[0.2\log(\bar{R}^v)\theta_8 + \log(\bar{R}^v)\right]$\\
$p_g^f(0)$ & $\num{50e3}\theta_3+\num{150e3}$\\
$K$ & $0.2\log(\bar{K})\theta_4 + \log(\bar{K})$\\
$W$ & $0.2\log(\bar{W})\theta_5 + \log(\bar{W})$ \\
$c_s^v$ & $0.2\log(\bar{c}_s^v)\theta_6 + \log(\bar{c}_s^v)$\\
$R^f$ & $0.2\log(\bar{R}^f)\theta_7 + \log(\bar{R}^f)$\\
$R^v$ & $0.2\log(\bar{R}^v)\theta_8 + \log(\bar{R}^v)$\\
$L^f$ & $0.2\log(\bar{L}^f)\theta_9 + \log(\bar{L}^f) $\\
$L^v$ & $0.2\log(\bar{L}^v)\theta_{10} + \log(\bar{L}^v)$\\\hline
\end{tabular}
\label{tab:MapleTransforms}
\end{table}

The inference parameters $\trv$ are related to the model parameters in \eqref{eq:MapleDae1}--\eqref{eq:MapleAlg5} using the transformations in Table \ref{tab:MapleTransforms}; variables with an overbar are default parameters taken from \cite{Ceseri2013} and shown in Table \ref{tab:MapleDefaults}.  Values for the remaining physical constants are listed in Table \ref{tab:MapleConstants}.


\begin{table}
\centering
\caption{Default values used to generate synthetic data and to scale the inference parameters  in the maple problem.}
\begin{tabular}{|c|c|c|p{7cm}|}\hline
Symbol & Value & Units & Description\\\hline
$\bar{s}_{gi}(0)$  & $0.7\bar{R}^f$ & $\si{\meter}$ & Initial location of gas-ice interface in fiber.\\
$\bar{s}_{iw}(0)$  &  $\bar{R}^f$ & $\si{\meter}$ & Initial location of ice-water interface in fiber.\\
$\bar{r}(0)$  &  $0.3\bar{R}^v$ & $\si{\meter}$ & Initial radius of vessel gass bubble.\\
$\bar{p}_g^f(0)$  &  $\num{200e3}$ & $\si{\pascal}$ & Initial gas pressure in fiber. \\
$\bar{K}$  & $\num{1.98e-14}$ & $\si{\meter\per\second}$ & Hydraulic conductivity of fiber-vessel wall.\\
$\bar{W} $ & $\num{3.64e-6}$ & $\si{\meter}$ & Thickness of fiber-vessel wall. \\ 
$\bar{c}_s^v$  &  $\num{58.4}$ & $\si{\mole\per\meter\cubed}$ & Sucrose concentration in vessel sap. \\
$\bar{R}^f$  & $\num{3.5e-6}$ & $\si{\meter}$ & Fiber radius. \\
$\bar{R}^v$ & $\num{2e-5}$ & $\si{\meter}$ & Vessel radius. \\
$\bar{L}^f$ & $\num{1e-3}$ & $\si{\meter}$ & Fiber length. \\
$\bar{L}^v$ &  $\num{5e-4}$ & $\si{\meter}$ & Vessel length.\\
\hline
\end{tabular}
\label{tab:MapleDefaults}
\end{table}

\begin{table}
\centering
\caption{Physical constants used in maple exudation model.}
\begin{tabular}{|c|c|c|p{5.5cm}|}\hline
Symbol & Value & Units & Description\\\hline
$\rho_i$ & $917$ & $\si{\kilogram\per\meter\cubed}$ & Density of water ice.\\
$\rho_w$ & $1000$ & $\si{\kilogram\per\meter\cubed}$ & Density of water. \\
$\lambda$ &   $\num{3.34e5}$ & $\si{\joule\per\kilogram}$ & Latent heat of fusion for water. \\
$R$ & $8.314$ & $\si{\joule\per\mole\per\kelvin}$ & Universal gas constant.\\
$g$ & $9.81$ & $\si{\meter\per\second\squared}$ & Acceleration due to gravity. \\
$\sigma$ & $0.0756$ & $\si{\newton\per\meter}$ & Surface tension of water. \\
$H$ & $0.0274$ & -- & Henry's constant for air and water. \\
$M_g$ & $0.0290$ & $\si{\kilogram\per\mole}$ & Molar mass of air.\\
$\kappa_w$ & $0.580$ & $\si{\watt\per\meter\per\kelvin}$ & Thermal conductivity of water.\\
$\kappa_g$ & $0.0243$ & $\si{\watt\per\meter\per\kelvin}$ & Thermal conductivity of air.\\
\hline
\end{tabular}
\label{tab:MapleConstants}
\end{table}






==> Paper4Arxiv 2/MyDefinitions.tex <==
%\pgfplotsset{colormap={myCmap}{rgb255=(247,251,255) rgb255=(222,235,247) rgb255=(198,219,239) rgb255=(158,202,225) rgb255=(107,174,214) rgb255=(66,146,198) rgb255=(33,113,181) rgb255=(8,81,156) rgb255=(8,48,107)}}

\newcommand{\real}{\mathbb{R}}
\newcommand{\Ex}{\mathbb{E}}
\def\argmin{\mathop{\mathrm{argmin}}}
\newcommand{\cov}{\mathbb{C}\mathrm{ov}}
\newcommand{\Var}[1]{\underset{#1}{\mathbb{V}\mathrm{ar}}}
\newcommand{\Varsimp}{\mathbb{V}\mathrm{ar}}
\newcommand{\eqd}{\buildrel d \over =}
\newcommand{\vnote}[1]{{\mbox{\boldmath ${#1}$}}}%vector
\newcommand{\setf}[1]{\mathcal{#1}}

\providecommand{\qed}{}

\newcommand{\algindent}{0.6cm}


\definecolor{nutsColor}{rgb}{0.9941,    0.7754,    0.6172}%
\definecolor{tmdrColor}{rgb}{0.5645,    0.7207,    0.8535}%
\definecolor{dramColor}{rgb}{0.84766,0.27734,0.00391}%


\newcommand{\trv}{\theta}
\newcommand{\rrv}{r}
\newcommand{\pd}{n}

\newcommand{\arrv}[1]{\tilde{\rrv}^{#1}}
\newcommand{\arrvs}[2]{\tilde{\rrv}^{#1,(#2)}}

\newcommand{\lebMeas}{\mu_{Leb}}
\newcommand{\td}{\pi} % unnormalized target density
\newcommand{\ntd}{\pi_n} % normalized target density
\newcommand{\rd}{p}
\newcommand{\crv}{\zeta}

\newcommand{\tmeas}{\mu_\trv}
\newcommand{\rmeas}{\mu_\rrv}
\newcommand{\qr}{q_\rrv}
\newcommand{\qt}{q_\trv} % proposal on target space
\newcommand{\emap}{T} % exact transport map
\newcommand{\demap}{{\nabla T}}

\newcommand{\imap}{{\widetilde{T}}} % inexact transport map
\newcommand{\dimap}{{\nabla \widetilde{T} }}

\DeclareMathOperator\erf{erf}
%\DeclareMathOperator\supp{supp}
% \DeclareMathOperator\arg{arg}
% \DeclareMathOperator\det{det}


\newcommand{\bspace}{\mathcal{B}(\real^D)} % the space of borel measurable sets

\newcommand{\tk}{P} % transition kernel

\newcommand{\mapp}{\gamma} % transition kernel
\newcommand{\mappa}{\bar{\mapp}}

\newcommand{\eqas}{\buildrel a.s. \over =}
\newcommand{\approxeqd}{\buildrel d \over \approx}

\newcommand{\nannerScale}{0.35}
\newcommand{\numSamps}{50}

\newcommand{\TraceWidth}{0.45\textwidth}
\newcommand{\TraceHeight}{0.2\textwidth}

%\newtheorem{definition}{Definition}
%\newtheorem{lemma}{Lemma}
%\newtheorem{theorem}{Theorem}


==> Paper4Arxiv 2/abstract.tex <==
\begin{abstract}
We introduce a new framework for efficient sampling from complex probability distributions, using a combination of transport maps and the Metropolis-Hastings rule. The core idea is to use deterministic couplings to transform typical Metropolis proposal mechanisms (e.g., random walks, Langevin methods) into non-Gaussian proposal distributions that can more effectively explore the target density. Our approach adaptively constructs a lower triangular transport map---an approximation of the Knothe-Rosenblatt rearrangement---using information from previous MCMC states, via the solution of an optimization problem. This optimization problem is convex regardless of the form of the target distribution. It is solved efficiently using a Newton method that requires no gradient information from the target probability distribution; the target distribution is instead represented via samples. Sequential updates enable efficient and parallelizable adaptation of the map even for large numbers of samples. We show that this approach uses inexact or truncated maps to produce an adaptive MCMC algorithm that is ergodic for the exact target distribution. Numerical demonstrations on a range of parameter inference problems show order-of-magnitude speedups over standard MCMC techniques, measured by the number of effectively independent samples produced per target density evaluation and per unit of wallclock time.

\end{abstract}


==> Paper4Arxiv 2/adaptivemcmc.tex <==
\section{Adaptive transport map MCMC}
\label{sec:adaptmcmc}
% With a sufficiently accurate map, Algorithm \ref{alg:fixedalg} provides a way to efficiently generate samples of the target density $\td(\trv)$.

Given more samples of the target distribution, we can construct a more accurate transport map, which in turn yields a more efficient map-accelerated proposal. Hence, we adaptively construct the the map $\imap$ as the MCMC chain progresses.

\subsection{Adaptive algorithm overview}
\label{sec:adaptmcmc:overview}

In our adaptive MCMC approach, we initialize the sampler with a simple map $\imap_0$ and update the map every $K_U$ s.pdf using the previous states of the MCMC chain. The map update uses these samples to define the optimization problem \eqref{eq:basicopt}, the solution of which yields a new map. This approach is conceptually similar to the adaptive Metropolis algorithm of \cite{Haario2001}.  In \cite{Haario2001}, however, previous states are used to update the covariance matrix of a Gaussian proposal; in the present case, previous states are used to construct a nonlinear transport map that yields more general non-Gaussian proposals. 

The most straightforward version of our adaptive algorithm would find the coefficients $\mapp_i$ for each component of the map by solving \eqref{eq:basicopt} directly.  However, when the number of existing samples $K$ is small or if the initial s.pdf of the chain mix poorly, the Monte Carlo sum in \eqref{eq:basicopt} will be a poor approximation of the true integral, producing maps that do not capture the structure of $\td$.  This is a standard issue in adaptive MCMC. One way to overcome this problem is to start adapting the map only after some initial exploration of the parameter space, i.e., after drawing a sufficient number of MCMC samples using the initial map $\imap_0$. A more efficient alternative, however, is to introduce a regularization term $g(\mapp_i)$ into the objective, allowing the map to start adapting much earlier. The purpose of this term is to ensure that the map does not prematurely collapse onto one region of the target space; such a collapse would make it difficult for the chain to efficiently explore the entire support of $\td$. Regularization yields the following modified objective:
\begin{equation}
\begin{aligned}
& \underset{\mapp_i}{\min}
& & g(\mapp_i) + \sum_{k=1}^{K}\left[  \frac12\imap^2_i(\trv^{(k)}; \mapp_i) - \log\left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}}\right]\\
& \text{s.t.}
& & \left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}} \geq  \lambda_{\text{min}}, \quad \forall k\in\{1,2,\ldots,K\} .
\end{aligned}\label{eq:regopt}
\end{equation}
In practice, we choose $g(\mapp_i)$ to prevent $\imap$ from deviating too strongly from the identity map, particularly when $K$ is small.  If additional problem structure such as the covariance of $\td$ were known, it could also be incorporated into the regularization term. But in the typical case, we use a simple quadratic penalty function centered on the coefficients of the identity map: letting $\mapp_i^{\text{Id}}$ denote the coefficients of the identity map, we put $g(\mapp_i) = k_R \|\mapp_i-\mapp_i^{\text{Id}}\|^2$ where $k_R$ is a user-defined regularization parameter. We have found that on most problems, small values of $k_R$ yield similar performance. (In the numerical examples below, we mostly set $k_R=10^{-4}$.)  Because we have discarded the $\frac{1}{K}$ coefficient scaling the Monte Carlo sum in \eqref{eq:regopt}, the second term of the objective overwhelms the regularization term as the number of samples grows, and the value of $k_R$ eventually becomes unimportant.

Lines 9--13 of Algorithm \ref{alg:adaptalg} show how we incorporate the map update into our adaptive MCMC framework.


\begin{algorithm}[h!]
\DontPrintSemicolon
\KwIn{Initial state $\trv_0$, initial vector of transport map parameters $\mappa_0$, reference proposal $q_\rrv( \cdot \vert \rrv^{(k)})$, number of s.pdf $K_U$ between map adaptations, total number of steps $L$.}
\KwOut{MCMC samples of the target distribution, $\left\{\trv^{(1)},\trv^{(2)},\ldots,\trv^{(L)}\right\}$}
Set state $\trv^{(1)} = \trv_0$\;
Set parameters $\mappa^{(1)} = \mappa_0$\;
\For{$k \gets 1 \ldots L-1$}{
Compute the reference state, $\rrv^{(k)} = \imap(\trv^{(k)}; \mappa^{(k)})$\;
Sample the reference proposal, $\rrv^\prime\sim q_\rrv(\cdot\vert\rrv^{(k)})$\;
Compute the target proposal sample, $\trv^\prime = \imap^{-1}(\rrv^\prime; \mappa^{(k)})$\;
Calculate the acceptance probability:
\[
\alpha = \min\left\{1, \frac{\td(\imap^{-1}(\rrv^\prime; \mappa^{(k)}))}{\pi(\imap^{-1}(\rrv^{(k)}; \mappa^{(k)}))} \frac{q_r\left(\rrv^{(k)}\vert\rrv^\prime\right)}{q_r\left(\rrv^\prime\vert\rrv^{(k)}\right)}\frac{\det[D\imap^{-1}(\rrv^\prime; \mappa^{(k)})]}{\det[D\imap^{-1}(\rrv^{(k)}; \mappa^{(k)})]}\right\}
\]\;
Set $\trv^{(k+1)}$ to $\trv^\prime$ with probability $\alpha$; else set $\trv^{(k+1)} = \trv^{(k)}$.\;
\eIf{$(k\bmod{K_U}) = 0$}{
\For{$i\gets 1 \textbf{ to } \pd$}{
Update $\mapp_i^{(k+1)}$ by solving (\ref{eq:regopt}) with $\left\{\trv^{(1)},\trv^{(2)},\ldots,\trv^{(k+1)}\right\}$\;
}
}{
$\mappa^{(k+1)} = \mappa^{(k)}$\;
}
}
\Return{\textrm{Target samples} $\left\{\trv^{(1)},\trv^{(2)},\ldots,\trv^{(L)}\right\}$}\;
\caption{MCMC algorithm with adaptive map}
\label{alg:adaptalg}
\end{algorithm}

\subsection{Sequential map updates}
\label{sec:adaptmcmc:mapupdate}

At first glance, updating the map every $K_U$ MCMC iterations might seem computationally taxing.  Fortunately, the form of the optimization problem in \eqref{eq:regopt} allows for efficient updates.  When $K_U$ is small relative to the current number of s.pdf $K$, the objective function in \eqref{eq:regopt} changes little between updates and the previous map coefficients provide a good initial guess for the new optimization problem.  Thus new optimal coefficients can be found in only a few Newton iterations, sometimes only one or two. As the timing results in Section \ref{sec:perf} show, even for long chains (large $K$), the advantage of using the map to define $q_{\trv,\bar{\mapp}}$ greatly outweighs the computational costs of sequential map updates.  

We also note that the optimization could be performed with stochastic approximation (SA) techniques \cite{Kushner2003,Andrieu2006}, in which case each map update would use only a portion of the chain, and would have a cost independent of $K$. Our tests with $K$ up to $\num{5e5}$ have shown SAA to be more efficient, but even longer chains might favor an SA approach.

% Moreover, when a polynomial expansion like \eqref{eq:polyexpand} is used to parameterize the map, we can simply add a new row to the matrices in \eqref{eq:basicopt2} at each iteration, avoiding redundant polynomial evaluations.  Combining this caching with efficient matrix-vector products makes evaluations of \eqref{eq:regopt} very efficient.  As the timing results in Section \ref{sec:perf} will show, with the help of these implementation s.pdf, the advantage of using the map to define $q_{\trv,\bar{\mapp}}$ greatly outweighs the additional cost of updating the map.
%
%\todo{What about ADMM and refs to Boyd? Are these useful and do you use it in the numerical examples? If so, we should mention it here. It would deepen this section.}

\subsection{Monitoring map convergence}
\label{sec:adaptmcmc:convg}
As the map in Algorithm \ref{alg:adaptalg} is adapted,  the pushforward of $\td$ through the map becomes closer to the reference Gaussian, and the best choice of reference proposal $q_\rrv(\rrv \vert \rrv^\prime)$ will evolve as well.  A small-scale random walk proposal may be appropriate at early iterations, but a larger and perhaps position-independent proposal may be advantageous as the map captures more of the target distribution's structure.  By monitoring the difference between $\tilde{\rd}$ \eqref{eq:referenceTarget} and the uncorrelated standard Gaussian density, we can adapt the reference proposal $q_\rrv$ to better explore the changing $\tilde{\rd}$.

To this end, it is important to have an indicator of the map's current accuracy. In the discussion following \eqref{eq:klexpr}, we noted that $\log \td - \log p \circ \imap - \log | \det \dimap |$ becomes a constant function of $\trv$ when an exact transformation \eqref{eq:measconst} between the target and reference is achieved. 
%If $\td$ is properly normalized, then this constant is in fact zero; more generally, it is the log of the normalizing constant of $\td$. In either case, 
A useful way to monitor the map's convergence is then to calculate the variance of this quantity,
\begin{equation}
\sigma^2_M = \Varsimp_{\trv} {\left[\log \td(\trv) -  \log p\left(\imap(\trv)\right) -\log \left | \det \dimap(\trv) \right | \right] } .
\label{eq:mapvar}
\end{equation}
A variance of zero indicates that the map is exact: $\tilde{\rd}$ is a standard Gaussian. 
% See \cite{Moselhy2011} for more information on the asymptotic behavior of $\sigma_M^2$.
Asymptotically, as $\sigma^2_M \rightarrow 0$, the KL divergence \eqref{eq:klexpr} becomes $2 \sigma^2_M$ \cite{Moselhy2011}. 

%The next section will describe one possible scheme for using $\sigma^2_M$ to adapt the proposal; others are certainly feasible.

% While not discussed in this paper, we want to acknowledge that $\sigma_M$ could be be used to tune other types of proposal as well, e.g., to adapt proposal variances or set weights in a Crank-Nicholson proposal \cite{Cotter2012}.

\subsection{Choice of reference proposal}
\label{sec:adaptmcmc:refprop}

Until now, we have left the choice of reference proposal $q_\rrv(\rrv^\prime \vert \rrv)$  rather open.  Indeed, any non-adaptive proposal, including both independence proposals and random walk proposals, could be used within our framework.  Figure \ref{fig:propTypes} shows some typical proposals on both the reference space and the target space.  In this section, we describe a few reference proposals that we will use in our numerical demonstrations, with particular attention to how they are implemented within the transport map framework. This selection is far from exhaustive, and is only intended to indicate how the transport map can dictate the choice of reference proposal.

\newcommand{\propScale}{0.22}
\begin{figure}[h]
\centering

\begin{subfigure}{0.24\textwidth}
\input{pics/mcmc/LocalMapReference.tex}
\caption{Local reference.}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\input{pics/mcmc/LocalMapBanana.tex}
\caption{Local Target.}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\input{pics/mcmc/GlobalMapReference.tex}
\caption{Global reference.}
\end{subfigure}
\begin{subfigure}{0.24\textwidth}
\input{pics/mcmc/GlobalMapBanana.tex}
\caption{Local target.}
\end{subfigure}

%\subfigure[Local target.]{\input{pics/mcmc/LocalMapBanana.tex}}
%\subfigure[Global reference.]{\input{pics/mcmc/GlobalMapReference.tex}}
%\subfigure[Global target.]{\input{pics/mcmc/GlobalMapBanana.tex}}

 \caption[Illustration of map-induced proposals.]{Example proposals in the reference space and the target space.  Plots of both $q_\rrv(\rrv^\prime \vert \rrv)$ and $q_\trv(\trv^\prime\vert\rrv)=q_\rrv(\rrv^\prime \vert \rrv) |D\imap(\trv^\prime)|$ are shown for local and independence (global) proposals. The black contours depict the target distributions while the colored contours illustrate the proposal densities.}
 \label{fig:propTypes}
 \end{figure}
 
\textbf{Metropolis-adjusted Langevin (MALA) proposal:}  Discretizing an appropriate Langevin equation yields a proposal of the form:
\begin{equation}
q_{\text{MALA}}(\rrv^\prime \vert \rrv) = \mathcal{N} \left( \rrv + \frac{(\Delta \tau)^2}{2} \nabla_{\rrv} \log \tilde{\rd}(\rrv), \, (\Delta \tau)^2 \, I \right),
\label{eq:malaprop}
\end{equation}
with a s.pdfize $(\Delta \tau)^2$ and a symmetric positive definite matrix $\Sigma$ \cite{Roberts1996}.  

\textbf{Delayed rejection proposals:} The delayed-rejection (DR) MCMC scheme of \cite{Mira2001} allows several proposals to be attempted during each MCMC step. With such a multi-stage proposal, we can try a larger or more aggressive proposal at the first stage, followed by more conservative proposals likely to produce accepted moves.  We use this scheme to define $q_\rrv(\rrv^\prime \vert \rrv)$ in two ways.  

Our first instantiation of DR employs a standard Gaussian as an independence proposal in the first stage, followed by a Gaussian random walk proposal in the second stage. Our motivation for this global-then-local strategy is the evolving nature of $\tilde{\rd}(\rrv)$.  Initially, $\tilde{\rd}(\rrv)$ will resemble the target density, which is more efficiently sampled by the random walk proposal; we need samples to be accepted in order to build a good map. As the map adapts, however, $\tilde{\rd}(\rrv)$ will approach a standard normal density, which can be efficiently explored by the position-independent first stage. DR naturally trades off between these alternatives.
% 
% 
% After many MCMC s.pdf, this density may become nearly Gaussian---in which case the independence proposal in the first stage could generate nearly independent samples.  On the other hand, we need many samples to build a good map and an independent Gaussian proposal will be inefficient during the early steps of the MCMC chain.  The random-walk second stage becomes most useful in this phase of the algorithm. Even when the first-stage proposal is rejected, the second stage will ensure that our sampler continues to explore the target space.  As $\imap$ begins to capture the structure in $\td$, the first stage of the proposal will be accepted more frequently and the mixing of the chain will improve.
Figure~\ref{fig:propTypes} illustrates the difference between local and independence proposals for a simple banana-shaped distribution.
%
Our second instantiation of DR employs two symmetric random-walk proposals, the first with a larger variance and the second with a smaller variance.
%Our motivation is the same as before: the larger proposal will be more effective for a more Gaussian $\tilde{\rd}$, while the smaller proposal will ensure that the chain explores the target space even when $\imap$ does not yet capture any of the structure in $\td$.  

%\textbf{Mixture proposals:} \textcolor{red}{[Remove this?]} An alternative to using the independence proposal in the delayed rejection framework above is to use it as one component of a mixture proposal. The second component of the proposal, as in delayed rejection, is a random walk.  With probability $w$, we draw a sample from the standard Gaussian and with probability $1-w$ we draw a sample from the local random walk. The key to making this method efficient is to choose the weight $w$ based on the map's current accuracy, i.e., how well the the map captures the target density $\td$.  Let $\hat{\sigma}_M^{2,{(k)}}$ be a Monte Carlo estimate of $\sigma^2_M$ \eqref{eq:mapvar} at the $k$th MCMC iteration.  We choose the mixture weights based on the following function
%\begin{equation}
%w = \frac{w_{\text{max}}}{1 + w_{\text{scale}}\hat{\sigma}_M^{2,{(k)}}}\label{eq:mixWeightFunc},
%\end{equation}
%where $w_{\text{max}}\in[0,1]$ and $w_{\text{scale}}\in[0,\infty)$ are tunable parameters.  Notice that %$w\rightarrow w_{\text{max}}$ as $\hat{\sigma}_M^{2,{(k)}}\rightarrow 0$; in other words,   
%% When the chain is mixing well  and $\hat{\sigma}_M^{2,{(k)}}$ is a good estimate of $\sigma_M^{(k)}$, this means that
%$w\rightarrow w_{\text{max}}$ as the map captures more of the structure in $\td$.  In practice, when the chain is not mixing properly, we find that the Monte Carlo estimate of $\hat{\sigma}_M^{2,{(k)}}$ might give an overly optimistic impression of the map's accuracy. We overcome this issue by always choosing $w_{\text{max}}<1$ (e.g., $0.9$) and by setting $N_U$ so that at least a few s.pdf are likely to be accepted between map updates.
%
%\todo{Technically speaking, since $w$ is being adjusted during the MCMC, the mixture approach is an adaptive proposal embedded within another adaptive proposal (controlled by the maps). Is this actually safe in practice, and does our theory apply here?}

%\section{Relationship to Geodesic MCMC}
%\label{sec:geomcmc}
%A class of differential geometric MCMC approaches was introduced by \cite{Girolami2011}.  These differential geometric approaches use a position specific metric to define a Riemannian manifold on which to perform MCMC.  At each point, the manifold captures some of the local correlation structure of the target distribution and allows to proposal to locally adapt to the target.   In the original work, \cite{Girolami2011} used the expected Fisher information metric to define the manifold.  However, as the authors are quick to point out, alternative metrics can also be used.  In fact, the map in our approach can be used to define such a metric.  On top of that, our numerical experiments suggest that moving along geodesics on this map-induced manifold is equivalent to moving linearly in the reference space.  Recall that geodesics are the shortest paths on a manifold.
%
%To derive the map-induced metric, consider the approximate map $\imap(\trv)$.  Now, let $J^{-1}(\rrv)=\dimap^{-1}(\rrv)$ be the Jacobian matrix of the inverse map evaluated at $\rrv$ and $J(\trv)=\dimap(\trv)$ be the Jacobian matrix of the forward map $\imap(\trv)$ evaluated at $\trv$.  A small change  $\delta \trv$ from $\trv$ in the target space corresponds to a small change $\delta \rrv = J(\trv) \delta \trv$ in the reference space.  The inner product $\delta \rrv^T\delta \rrv$ can then be written in term of $\trv$ as 
%\begin{equation}
%\delta \rrv^T\delta \rrv = \delta \trv^T  \left( J(\trv)^T J(\trv)\right) \delta \trv
%\end{equation}
%This inner product defines a position-dependent metric defined by the matrix:
%\begin{equation}
%G^M(\trv) = J(\trv)^T J(\trv)\label{eq:metric}
%\end{equation}  
%Since $|\mbox{det }J|\geq d_{min}$ by our monotonicty constraint, $G^M$ is guaranteed to be a symmetric positive definite matrix.  This metric defines a manifold on the target space much like the expected Fisher information metric used in \cite{Girolami2011}.  
%
%Not only does the map define a metric, but from our observations it seems that evaluating the map is equivalent to moving along a geodesic on the manifold.  For illustration, consider a simple ``banana" shaped density defined by the following quadratic transformation:
%\[
%\left[\begin{array}{c}\trv_1\\\trv_2\end{array}\right] = \emap^{-1}(\rrv) =  \left[\begin{array}{l}\rrv_1 \\ \rrv_2 -2(\rrv_1^2 + 1)\end{array}\right]  
%\]
%where $\rrv_1$ and $\rrv_2$ are (as usual) IID Gaussian random variables.  Figure \ref{fig:geodesiccomp} shows a comparison of Geodesic paths computed using (\ref{eq:metric}) and linear paths on the reference space pushed through the map.  Let $w_g(t)$ be the geodesic path, parameterized by $t\in[0,1]$, between $w(0)$ and $w(1)$ and $w_m(t)$ be the another path between the same two points defined by:
%\begin{equation}
%w_m(t) = \imap^{-1}\left(\imap(w(0)) + t \left[\imap(w(1))-\imap(w(0))\right]\right)\label{eq:mapPath}
%\end{equation}
%Figure \ref{fig:geodesiccomp} compares $w_m(t)$ and $w_g(t)$ for 15 different values of $w(1)$ and $w(0)=[0,0]^T$.  In this simple example, the mapped paths from (\ref{eq:mapPath}) and the geodesic paths look identical, which seems to imply that our transport maps are also time one geodesic flows on a Riemannian manifold.  A more theoretical analysis of this observation could provide a more rigorous connection between our map-based MCMC, geodesic MCMC, and Riemannian geometry.
%
%\begin{figure}
%\centering
%
%\subfigure[Geodesic paths, $w_g(t)$, constructed on the manifold defined by $G^M(\trv)$ in (\ref{eq:metric}).]{
%\centering
%\begin{tikzpicture}[scale=0.85]
%\input{pics/GeodesicPaths.tex}
%\end{tikzpicture}
%}\subfigure[Map paths, $w_m(t)$, constructed using (\ref{eq:mapPath}).]{
%\centering
%\begin{tikzpicture}[scale=0.85]
%\input{pics/MapPaths.tex}
%\end{tikzpicture}
%}
%
%\caption{Comparison of 15 different geodesic paths and mapped paths.   Paths are shown in black.  The Geodesic paths were constructed by integrating a Hamiltonian system describing the geodesic. An initial momentum $p$ was used and a leap frog integrator was used until some finishing time $t_f$.  On the other hand, the map paths are evaluations of $\imap^{-1}(tp) \quad \forall t\in(0,t_f)$ for the same 15 initial momentums $p$ used for the Geodesic plot.  Colored contours of the target density $\td(\trv)$ are shown in the background.}
%\label{fig:geodesiccomp}
%\end{figure}
%


==> Paper4Arxiv 2/conclusions.tex <==
\section{Conclusions}
\label{sec:conc}
% What we did, in essence.
% Why it's efficient.
% Where this method can and should be applied.
% costs/overhead, and overall performance

% Extensions:
% - parallelism
% - other map bases
% 
% Extensions, for high dimensions:
% - adaptive approximation
% - nonparametric approaches
% - connections with geometric methods: metric

We have introduced a new MCMC approach that uses transport maps to accelerate sampling from challenging target distributions. Our approach adaptively constructs nonlinear transport maps from MCMC samples, via the solution of a convex and separable optimization problem. From one perspective, the resulting maps transform the target to a reference distribution that is increasingly Gaussian and isotropic, and hence easier to sample. From a complementary perspective, the maps transform simple proposal mechanisms into non-Gaussian proposals on the target. Our maps are by construction invertible and continuously differentiable functions between the reference and target spaces, and hence they allow broad flexibility in choosing reference-space MCMC proposals. Yet building the maps themselves requires no derivative information from the target distribution. 

The efficiency of our approach is primarily a result of capturing nonlinear dependencies and non-Gaussian structure in the posterior and, when possible, exploiting this knowledge with global independence proposals (e.g., TM+DRG).  Of course, sequentially updating the transport map introduces an additional computational cost, which may become important in simple problems. As shown in the BOD example, however, our methods can be more efficient on strongly non-Gaussian problems, even when the target density is trivial to evaluate. On more complex posteriors, as in the ODE and DAE examples of Section~\ref{sec:perf:predprey} and \ref{sec:perf:maple}, the efficiency gains can be even more significant, both in terms of effective sample size per posterior evaluation and effective sample size per unit of wallclock time. It is also important to point out that our current implementation does not exploit the many levels of parallelism afforded by the map construction algorithm: solution of the optimization problem \eqref{eq:regopt} can made embarrassingly parallel over parameter dimensions, and additional parallelism can be introduced over samples.\footnote{Our implementation is freely available in MUQ \cite{MUQ}. This work used commit 7417f35 from MUQ's git repository.}

% derivatives!!!
% no particular structure: sMMALA,


% Extensions:
% - parallelism
% - other map bases
% 
% Extensions, for high dimensions:
% - adaptive approximation
% - nonparametric approaches
% - connections with geometric methods: metric

While the present work used polynomials to represent the transport map, this is not an essential aspect of the framework. In fact, the optimization problem for the map coefficients in \eqref{eq:regopt} will be unchanged for any map representation that is linear in the coefficients; we have experimented with other bases, e.g., radial basis functions, to good effect. 
% When the target density is expensive to evaluate, any parameterization of the transport map will help capture some of the target structure and yield improved sampling. 
%
Performance can be enhanced by an appropriate choice of basis, however, and future work will explore adaptive basis selection strategies. These will be particularly important for extending the transport map approach to higher-dimensional problems, where a more parsimonious choice of basis (versus the total-order bases used here) will be required. Recent results on the sparsity of triangular transports, and the decomposability of more general transports, may be useful in this regard \cite{Spantini2017}. Other methods for approximating the map, perhaps even nonparametric approaches, may also useful. We also note that the transport map defines a Riemannian metric on the parameter space, locally given by $(\dimap(\trv))^\top (\dimap(\trv))$. This suggests links between map-accelerated sampling and differential geometric MCMC methods, which we plan to explore.


% This includes other choices such as radial basis functions.  Polynomials were used here primarily for their global smoothness properties, their properties are well understood, and they have long been used in the uncertainty quantification community (e.g., \cite{Marzouk2009} and \cite{LeMaitre2010}).  Even if using polynomials, choosing the basis for a specific problem (instead of the total order limited polynomials used here) is likely to decrease the computational cost of constructing the map or increase the descriptive power of the map.  In either case, users are likely to see increased performance.

% We should also note that extending this work to higher dimensional problems will require a more frugal choice of polynomial basis than the total order limited polynomials used here.  Also, on high dimensional problems, combining more approximate maps with proposal mechanisms that exploit derivative information (such as HMC or MMALA) is also likely to improve convergence.  When the target density is expensive to evaluate, any parameterization of the transport map will help capture some of the target structure and yield improved sampling. Further investigation into the relationship between map-accelerated MCMC (the map Jacobian defines a local metric given by $\dimap(\trv)^\top \dimap(\trv)$) and differential geometric MCMC techniques could also be beneficial in the high dimensional setting.

% Save this, to reduce length!
%
% In conclusion, combining inexact transport maps with standard proposal mechanisms provides a novel new framework for adaptive (or standard) MCMC that can lead to significant performance improvements.  We believe this new framework is valuable tool to consider as the statistical community continues to invent and tackle ever more challenging sampling problems.


==> Paper4Arxiv 2/convergence.tex <==
\section{Convergence analysis}
\label{sec:convergence}
This section investigates conditions under which our adaptive algorithm yields an ergodic chain. Proofs of the lemmas are deferred to Appendix \ref{sec:detailedConvergence}.
%We first build intuition by analyzing the fixed-map algorithm (Algorithm \ref{alg:adaptalg} without the map update), and then establish conditions for convergence of the adaptive algorithm. 

\subsection{The need for bounded derivatives}
\label{sec:convergence:bounds}
%It is important to understand how the transport map affects the convergence properties of the reference MCMC chain. To illustrate this question, 
Consider a random walk proposal on the reference space, $q_\rrv(\rrv^\prime | \rrv) = N(\rrv, \sigma^2 I)$ with some fixed variance $\sigma^2$.  For illustration, assume that the target density is a standard normal distribution: $\td(\trv) = N(0,I)$.  The RWM algorithm is geometrically ergodic for any density satisfying the following two conditions (see Theorem 4.3 of \cite{Jarner2000}):
\begin{equation}
\limsup_{\| \trv \|\rightarrow \infty} \frac{\trv}{\| \trv \|} \cdot \nabla\log\td(\trv) = -\infty,\label{eq:superLight}
\end{equation}
and
\begin{equation}
\lim_{\| \trv \|\rightarrow \infty} \frac{\trv}{\| \trv \|} \cdot \frac{\nabla\log\td(\trv)}{\|\nabla\log\td(\trv)\|} < 0.\label{eq:curveCond}
\end{equation}
Densities that satisfy \eqref{eq:superLight} are called super-exponentially light.
   It is easy to show that our example Gaussian density satisfies these conditions.  In Algorithm \ref{alg:adaptalg}, however, instead of applying the RWM proposal to $\td$ directly, we apply the RWM proposal to the map-induced density in \eqref{eq:referenceTarget}.
% \begin{equation} \tilde{\rd}(\rrv) = \td(\imap^{-1}(\rrv))\left|\mbox{det} \dimap^{-1}(\rrv)\right|.
% \end{equation}
If the conditions in (\ref{eq:ubMap}) are not satisfied, we can show that even when $\td$ is Gaussian, any monotone {polynomial} map with degree greater than one results in a density $\tilde{\rd}(\rrv)$ that is no longer super-exponentially light.  For example, let $\imap$ have a maximum polynomial degree of $M>1$, with $M$ odd.  Then:
\begin{eqnarray}
\limsup_{\| \rrv \|\rightarrow \infty} \frac{\rrv}{\| \rrv \|} \cdot \nabla\log\tilde{\rd}(\rrv) &=& \limsup_{\| \rrv \|\rightarrow \infty}\frac{1}{\|r\|}\sum_{i=1}^\pd r_i \left(\frac{\partial \imap^{-1}_i}{\partial \rrv_i}\right)^{-1}\frac{\partial^2 \imap^{-1}_i}{\partial \rrv_i^2} \nonumber \\
&=&\limsup_{\| \rrv \|\rightarrow \infty}\frac{\pd}{\|r\|}\left(\frac{1}{M}-1\right)= 0 .\label{eq:zeroexplight}
\end{eqnarray}
%
%\begin{eqnarray}
%\limsup_{\| \rrv \|\rightarrow \infty} \frac{\rrv}{\| \rrv \|} \cdot \nabla \log\td(\imap^{-1}(\rrv))  & = & \limsup_{\| \rrv \|\rightarrow \infty} \frac{\rrv}{\| \rrv \|} \cdot \nabla\left[-0.5\rrv^{2/M}\right]\\
%& = & \limsup_{\| \rrv \|\rightarrow \infty} \frac{\rrv}{\| \rrv \|} \cdot \left[-\frac{1}{M}\rrv^{2/M-1}\right]\\
%&= & \limsup_{\| \rrv \|\rightarrow \infty} -\frac{1}{M}\frac{\rrv^{2/M}}{\| \rrv \|}\\
%&= & 0
%\end{eqnarray}
%
Clearly, the map-induced density is not super-exponentially light.  We have therefore jeopardized the geometric ergodicity of our sampler on a simple Gaussian target.  Additional restrictions on the map are needed to ensure convergence. 

The loss of geometric ergodicity in (\ref{eq:zeroexplight}) is due to the unbounded derivatives of nonlinear polynomial maps, which do not satisfy (\ref{eq:dUB}). Unbounded derivatives of $\imap$ imply that $\imap^{-1}$ has derivatives that approach zero as $\| \rrv \|\rightarrow \infty$, which leads to (\ref{eq:zeroexplight}).  More intuitively, without an upper bound on their derivatives, polynomial maps move too much weight to the tails of $\tilde{\rd}$.  In the next section, we show that the conditions in \eqref{eq:dUB} ensure the ergodicity of Algorithm \ref{alg:adaptalg}, even with map adaptation.

\subsection{Convergence of the adaptive algorithm}
Our goal in this section is to show that the adaptive Algorithm \ref{alg:adaptalg} produces samples that can be used in Monte Carlo approximations.  We thus need to show that Algorithm \ref{alg:adaptalg} is ergodic for the target density $\td(\trv)$.  

Assume that the target density is finite, continuous, and super-exponentially light.  (Note that certain densities which are not super-exponentially light can be transformed to super-exponentially light 
densities using the techniques from \cite{Johnson2012}.) Also assume that the reference proposal $q_\rrv(\rrv^\prime \vert \rrv)$ is Gaussian with bounded mean.
% (note that RWM proposals and truncated MALA proposals fall into this category).  
Furthermore, let $\Gamma$ be the space of the map parameters $\bar{\mapp}$ such that $\imap(\trv;\bar{\mapp})$ satisfies the bi-Lipschitz condition given by (\ref{eq:dUB}).

The map at iteration $k$ of the MCMC chain is defined by the coefficients $\bar{\mapp}^{(k)}$.  Let $\tk_{\bar{\mapp}^{(k)}}$ be the transition kernel of the chain at iteration $k$, constructed from the map $\imap(\trv;\bar{\mapp}^{(k)})$, the target space proposal in (\ref{eq:mapprop}), and the Metropolis-Hastings kernel:
\begin{equation} 
\tk_{\bar{\mapp}^{(k)}}(\trv,\mathcal{A}) = \int_{\mathcal{A}} \left (
  \alpha(\trv^\prime, \trv)q_{\trv,\bar{\mapp}^{(k)}}(\trv^\prime |
  \trv) +\left(1-r(\trv)\right)\delta_\trv(\trv^\prime) \right ) d\trv^\prime \label{eq:mhkernel}.
\end{equation} 
Here  $q_{\trv,\bar{\mapp}^{(k)}}$ is the map-induced proposal density from 
(\ref{eq:mapprop}),  $\alpha(\trv^\prime, \trv)$ is the acceptance probability 
defined in (\ref{eq:basicmh}), and $r(\trv) = \int \alpha(\trv^\prime, \trv) 
q_{\trv,\bar{\mapp}^{(k)}}(\trv^\prime | \trv) d\trv^\prime$.   Now, following 
\cite{Roberts2007} and \cite{Bai2009}, we can establish the ergodicity of our adaptive 
algorithm by showing that it satisfies two conditions: diminishing adaptation 
and containment. Diminishing adaptation is defined as follows:

\vspace{0.3cm}
\begin{definition}[Diminishing adaptation]\label{def:dim}
For any starting point $x^{(0)}$ and initial set of map parameters
$\bar{\mapp}^{(0)}$, a transition kernel $\tk_{\bar{\mapp}^{(k)}}$
satisfies the diminishing adaptation condition when
\begin{equation}
\lim_{k\rightarrow \infty}\sup_{x \in \real^\pd}\left\| \tk_{\bar{\mapp}^{(k)}}(x,\cdot) - \tk_{\bar{\mapp}^{(k+1)}}(x,\cdot)\right\|_{TV} = 0 \quad\text{  in probability}
\end{equation}
where $\|\cdot\|_{TV}$ denotes the total variation norm.  
\end{definition}
\vspace{0.3cm}

Instead of working with the containment condition directly (see \cite{Bai2009} or \cite{Roberts2007}), we will show that our adaptive MCMC algorithm instead satisfies the simultaneous strongly aperiodic geometric ergodicity (SSAGE) condition.

\vspace{0.3cm} 
\begin{definition}[SSAGE]
\label{def:ssage}
Simultaneous strongly aperiodic geometric ergodicity (SSAGE) is the condition that there exist a measurable set $C\in \bspace$, a drift function $V:\real^\pd\rightarrow [1,\infty)$, and scalars $\delta>0$, $\lambda<1$, and $b<\infty$ such that $\sup_{x\in C} V(x) < \infty$ and the following two conditions hold:
\begin{enumerate}
\item \emph{(Minorization)} For each vector of map parameters $\bar{\mapp}\in\Gamma$, there is a probability measure $\nu_{\bar{\mapp}}(\cdot)$ defined on $C\subset \real^\pd$ with $\tk_\mapp(x,\cdot)\geq \delta \nu_{\bar{\mapp}}(\cdot)$ for all $x\in C$.
\item \emph{(Simultaneous drift)} $\int_{\real^\pd} V(x) \tk_{\bar{\mapp}}(x,dx) \leq \lambda V(x) + b I_C(x)$ for all $\bar{\mapp}\in\Gamma$ and $x\in\real^\pd$.
\end{enumerate}
\end{definition}
 \vspace{0.3cm}
 
By Theorem 3 of \cite{Roberts2007}, SSAGE ensures the containment condition.  The following three lemmas establish diminishing adaptation and SSAGE.  % Proofs of these lemmas are deferred to Appendix \ref{sec:detailedConvergence}. 
 In the following, let $C=B(0,R_C)$ be a ball of radius $R_C>0$ and let $V(x) = k_v\td^{-\alpha}(x)$ for some $\alpha\in(0,1)$ and $k_v = \sup_x\td^{\alpha}(x)$.   Also, assume that $\td(x)>0$ for all $x\in C$.  For this choice of $V(x)$ and our assumption that $\td(x)>0$ for $x\in C$, we have that $\sup_{x\in C} V(x) < \infty$. 
 
Because the reference proposal is Gaussian with bounded mean, we can find two 
scalars $k_1$ and $k_2$, and two zero-mean Gaussian densities $g_1$ and 
$g_2$, such that the reference proposal is bounded as
 \begin{equation}
 k_1g_1(\rrv^\prime-\rrv)\leq q_\rrv(\rrv^\prime | \rrv) \leq k_2g_2(\rrv^\prime - \rrv)\label{eq:qrBounds}.
 \end{equation}
The bounds in (\ref{eq:dUB}) then imply that the target space proposal can also be bounded.  This result is captured in Lemma \ref{lem:propBnds}.

\vspace{0.3cm}
  \begin{lemma}[Bounded target space proposal]
  \label{lem:propBnds}
 For any map coefficients $\bar{\mapp} \in \Gamma$, the map-induced proposal $q_{\trv,\bar{\mapp}}(\trv^\prime | \trv)$ is bounded as
 \begin{equation}
 k_L g_L (\trv^\prime-\trv)\leq q_{\trv,\bar{\mapp}}(\trv^\prime | \trv) \leq k_Ug_U(\trv^\prime - \trv)\label{eq:qtBounds},
 \end{equation}
   where $k_L = k_1 \lambda_{\mathrm{min}}^\pd$, $k_U = k_2 \lambda_{\mathrm{max}}^\pd$,  $g_L(x) = g_1( \lambda_{\mathrm{max}} x)$, and $g_U(x) = g_2( \lambda_{\mathrm{min}} x)$.  
   \end{lemma}
   \vspace{0.3cm}

The upper and lower bounds in (\ref{eq:qtBounds}) are key to our proof of convergence.  In fact, with these bounds, the proofs of Lemma \ref{lem:minor} and Lemma \ref{lem:drift} below closely follow the proof of Proposition 2.1 in \cite{Atchade2006}.  Again, proofs of these results are left to the appendix.
  
 \vspace{0.3cm}
\begin{lemma}[Diminishing adaptation of Algorithm \ref{alg:adaptalg}]
\label{lem:dimAdapt}
Let the map parameters $\bar{\mapp}$ be restricted to a compact subset of $\Gamma$.  Then, the sequence of transition kernels defined by the update step in lines 9--13 of Algorithm \ref{alg:adaptalg} satisfies the diminishing adaptation condition. 
\end{lemma}
\vspace{0.3cm}

\begin{lemma}[Minorization condition for Algorithm \ref{alg:adaptalg}]
\label{lem:minor}
There is a scalar $\delta$ and a set of probability measures $\nu_{\bar{\mapp}}$ defined on $C$ such that $\tk_{\bar{\mapp}}(x,\cdot) \geq \delta \nu_{\bar{\mapp}}(\cdot)$ for all $x\in C$ and $\bar{\mapp}\in\Gamma$.
\end{lemma}
\vspace{0.3cm}
% \begin{proof}[Sketch of proof for Lemma \ref{lem:minor}]
% Let $\tau$ be the minimum acceptance rate over all $x,y\in C$ and over all map-induced proposals defined by
% \[
% \tau = \inf_{\bar{\mapp}\in\Gamma} \inf_{x,y \in C} \min\left\{1, \frac{\td(y) q_{\trv,\bar{\mapp}}(x | y)}{\td(x) q_{\trv,\bar{\mapp}}(y |x)}\right\}.
% \]
% Notice that $\tau>0$ because
% \[
% \td(y) q_{\trv,\bar{\mapp}}(x | y) \geq \td(y) k_{L}g_L(x-y)>0 \quad \forall x,y\in C.
% \]  
% Now, using the Metropolis-Hastings kernel in (\ref{eq:mhkernel}) and the lower bound in (\ref{eq:qtBounds}), we have 
% \[
% \tk_{\bar{\mapp}}(x,dy) \geq \tau k_L g_L(x-y) dy.
% \]
% Define a new probability density $g_{C}(y) = \frac{\inf_{x\in C} 
% g_L(x-y)}{\int_{\real^\pd} \inf_{x\in C}g_L(x-y) dy }$.  Because $g_L$ is a 
% Gaussian density and thus nonzero over $C$, $g_{C}(y)$ is a valid probability 
% density.  Define the scalar $k_{C} = k_L \int_{\real^\pd} \inf_{x\in C}g_L(x-y) 
% dy$ and set $\delta = \tau k_{C}$.  Notice that $\tk_{\bar{\mapp}}(x,dy)\geq 
% \tau k_{C} g_L(y) dy$.  Now define the measure \[\nu_{\bar{\mapp}}(A) = \nu(A) = 
% \frac{\int_{A\cap C} g_{C}(z) dz}{\int_{C} g_{C}(z) dz}\]  This is a nontrivial 
% probability measure defined over $C$.  Furthermore, we have 
% $\tk_{\bar{\mapp}}(x,\cdot) \geq \delta \nu(\cdot)$ and the minorization 
% condition is satisfied.  A more detailed proof is provided in Appendix 
% \ref{sec:detailedConvergence}.
% \end{proof}

\begin{lemma}[Drift condition for Algorithm \ref{alg:adaptalg}]
\label{lem:drift}
For all points $x\in \real^\pd$ and all feasible map parameters $\bar{\mapp}\in\Gamma$, there are scalars $\lambda$ and $b$ such that $\int_{\real^\pd} V(x) \tk_{\bar{\mapp}}(x,dx) \leq \lambda V(x) + b I_C(x)$
\end{lemma}
\vspace{0.3cm}

% \begin{proof}[Sketch of proof for Lemma \ref{lem:drift}]
% Using the bounds in (\ref{eq:qtBounds}), we can follow the proof of  Lemma 6.2 in \cite{Atchade2006} to show that the following two conditions hold:
% \[
% \sup_{x\in\real^\pd}\sup_{\bar{\mapp}\in\Gamma} \frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}(x,dy)}}{V(x)} <\infty
% \]
% and
% \[
% \limsup_{\|x\|\rightarrow\infty} \sup_{\bar{\mapp}\in\Gamma}\frac{\int_{\real^\pd} V(y) P_{\bar{\mapp}}(x,dy)}{V(x)} < 1.
% \]
% With these two conditions in hand, Lemma 3.5 of \cite{Jarner2000} gives the 
% existence of $\lambda$ and $b$ needed to satisfy the drift condition.  
% Further details are provided in Appendix 
% \ref{sec:detailedConvergence}.
% \end{proof}

\noindent With Lemmas \ref{lem:dimAdapt}--\ref{lem:drift} in hand, Theorem \ref{thm:ergodic} finally yields the ergodicity of our adaptive algorithm.
\vspace{0.3cm}

\begin{theorem}[Ergodicity of Algorithm \ref{alg:adaptalg}]
\label{thm:ergodic}
Algorithm \ref{alg:adaptalg} is ergodic for the target distribution $\td(\trv)$ 
when $\bar{\mapp}$ is constrained to a compact set within which $\imap(\trv;\bar{\mapp})$ is 
guaranteed to satisfy (\ref{eq:dUB}) for all $\trv \in \real^\pd$.
\end{theorem}
\begin{proof} %[Proof of Theorem \ref{thm:ergodic}]
Lemmas \ref{lem:minor} and \ref{lem:drift} ensure that SSAGE is satisfied, which subsequently ensures containment.  The diminishing adaptation property from Lemma \ref{lem:dimAdapt} combined with SSAGE implies ergodicity by Theorem 3 of \cite{Roberts2007}.
\end{proof}



==> Paper4Arxiv 2/intro.tex <==
\section{Introduction}
\label{sec:intro}

Markov chain Monte Carlo (MCMC) algorithms provide an enormously flexible approach for sampling from complex target probability distributions, using only evaluations of an unnormalized probability density \cite{Gelman2003, RobertBook2004, Liu2004, Brooks2011}. Within this general framework, the Metropolis-Hastings algorithm \cite{Metropolis1953,Hastings1970} is one of the most broadly applicable and well studied sampling strategies.
% methods for constructing an appropriate Markov process.  
%
It combines a simple proposal distribution with an accept/reject step to create the transition kernel for a Markov chain that has the desired target as its stationary distribution. Under some additional technical conditions on the proposal $q_\trv$ and target density $\td$, the Markov chain is also ergodic \cite{Roberts2004}.

This paper introduces a new approach to the design of Metropolis-Hastings algorithms, based on the adaptive construction of \textit{transport maps} between the target probability distribution and a simple reference distribution. These maps are monotone and typically nonlinear transformations of the target distribution that render it easier to sample, much like a preconditioner expedites the solution of a linear system. To put our approach in context, we first recall some challenges underlying MCMC sampling and current methods for addressing them.

% progressively % ``Gaussianize'' it or otherwise 

% With this in mind, we introduce a new family of proposals that use nonlinear variable transformations called transport maps to globally approximate the target density.  While our approach has a uniquely general structure that can yield order of magnitude performance increases (see Section \ref{sec:perf}), many other proposal mechanisms, such as those outlined below, have been developed with similar goals in mind.

%% talk about other proposal mechanisms here, mostly NUTS, DRAM, Gaussian Mixture Ind., and Riemannian Manifold.
Effective MCMC proposal mechanisms seek to make successive iterates of the Markov chain as independent as possible. When estimating an expectation over the target distribution, efficient ``mixing'' in this sense reduces the variance of estimates computed from the MCMC samples. A useful intuition is that effective MCMC proposals aim to approximate the target distribution at least locally (e.g., in the case of random-walk Metropolis or Langevin proposals) or perhaps globally (e.g., in the case of Metropolis independence samplers). Consider, for example, a Gaussian proposal density centered at the current state of the chain, as in a random-walk Metropolis algorithm. The adaptive Metropolis scheme of \cite{Haario2001} sequentially updates the covariance of this proposal in order to reflect the covariance of $\td$. In a similar fashion, \cite{Atchade2006} uses the empirical covariance of the target to scale proposals in a Metropolis-adjusted Langevin algorithm (MALA), which also uses the gradient of $\td$ to push the proposal mean towards regions of higher target density.

Many other MCMC algorithms use local derivative information to improve sampling 
of the target distribution. Hamiltonian Monte Carlo methods (HMC), as in 
\cite{Neal2011} and \cite{Hoffman2011}, propose samples via trajectories of a 
Hamiltonian dynamical system defined on an augmented state space. Computing 
these trajectories requires many evaluations of the gradient of the target 
density, but can produce large s.pdf that have high acceptance probability. The 
stochastic Newton method of \cite{Martin2012} uses higher-order derivative 
information, in the form of approximate Hessians of the local 
log-posterior, to scale a Gaussian proposal in high dimensions. The 
geometrically-motivated approach of \cite{Girolami2011} also uses 
higher-order derivative information to define a local metric for both 
Langevin proposals and Hamiltonian dynamics on a Riemannian manifold.
%
Contrasting with these schemes but also related to our work are adaptive Metropolis independence samplers \cite{Andrieu2006}, which 
%do not require derivatives of the target density but instead
construct a global approximation of the target using, for example, Gaussian mixtures. This approximation is updated recursively from past MCMC samples using a stochastic approximation scheme.

The theory of optimal transport has a rich history that is somewhat separate 
from stochastic simulation and MCMC. The notion of an optimal transport map 
dates back to \cite{Monge1781}, who sought a deterministic coupling between 
(probability) measures that is optimal in the sense of minimizing an expected 
transport cost. This cost is defined by a function $c(\theta, r)$ 
that can be interpreted as the cost of transporting one unit of mass from 
$\theta$ to $r$. A relaxation of the Monge problem to more general couplings 
was introduced by Kantorovich \cite{Kantorovich1942, Vershik2013}; yet under 
certain conditions, a minimizer of the Kantorovich formulation also solves the 
Monge problem, i.e., is an optimal transport map. For a contemporary development 
of this subject, see \cite{Villani2009, Villani2003} and \cite{Rachev1998}. 
%
Optimal transport between discrete measures has been used for Bayesian inference in \cite{Reich2013}, where the solution of a discrete assignment problem yields a consistent ensemble transformation scheme to replace resampling, in the context of a Bayesian filter. This problem differs from those considered here, however, as we focus on transport between continuous probability measures. % and inference problems that are not recursive. 
%
\cite{Moselhy2011} introduced the idea of continuous transport maps that characterize the Bayesian posterior distribution as a pushforward of the prior distribution. In this formulation, the transport map is used to generate independent samples from a distribution that in principle can be made arbitrarily close to $\td$. However, constructing sufficiently accurate maps can be computationally taxing.
% and, for complex target distributions, requires attention to the basis representation of the map 
% and for complex target distributions, require adaptive parameterizations 
The implicit sampling approach of \cite{chorin2009implicit,Chorin2010,Morzfeld2012} and the randomize-then-optimize approach of \cite{Bardsley2014} compute the action of certain transport maps sample-by-sample, without representing the maps explicitly. But these samples do not come from $\td$ and thus require reweighing in order to represent the target. 
% Both of these approaches involve optimization problems where $\td$ appears in the objective, and thus require access to gradients of $\td$. 
Implementing either of these approaches requires access to gradients of $\td$. %\todo{Check the prev discussion!}

In this paper, we will use \textit{approximate} transport maps to achieve \textit{exact} sampling from the target distribution, by integrating % [[explicitly parameterized?]]
transport maps with MCMC. We \textit{reverse} the direction of the maps computed in \cite{Moselhy2011}, and adaptively construct our maps (now from the target to a simple reference distribution)
by solving an optimization problem based on MCMC samples. We will show that the optimization problem has a remarkably simple structure: it is convex regardless of the form of the target distribution and separable across dimensions of the parameter space; it also affords substantial opportunities for parallel computation and efficient sequential updating.  Moreover, computing derivatives of the optimization objective requires no derivative information from the target probability density.  We will analyze the scheme from the theoretical perspective of adaptive MCMC, allowing us to establish ergodicity of the resulting chain.
%
The transport map constructed in this way aims to represent the entire target distribution as the pullback of a Gaussian reference measure, and in that sense our approach is a global one. Unlike adaptive Metropolis independence samplers, however, we approximate the target density not by choosing from a particular family of densities, but by building an invertible transformation between the target distribution and a reference distribution. Critically, this structure enables us to use both local proposals and global/independence proposals, and to transition naturally between the two as the transport map becomes more accurate. The transport map is not tied to any particular type of MCMC proposal; it instead provides a framework for improving many standard proposal schemes.
% (e.g., zero-mean random walk, HMC, or MALA).


% outline of paper here 
The remainder of this paper is organized as follows. Section~\ref{sec:maps} will provide relevant background on transport maps and explain how suitable maps can be constructed from samples. Section~\ref{sec:mapmcmc} will formulate the map-based MCMC approach, while Section~\ref{sec:adaptmcmc} will introduce adaptive strategies. A theoretical convergence analysis is provided Section~\ref{sec:convergence}. Section~\ref{sec:perf} compares the performance of map-based MCMC with that of existing state-of-the-art samplers on a range of test problems.


%
%\subsection{Mathematical setting and assumptions}
%\label{sec:intro:math}
%Before we get into the algorithmic details of our approach, this section will set the mathematical stage for what is to come.  Our ultimate goal is to generate samples of a random variable $\trv$ with $\pd$ dimensions. This random variable is defined on a suitable probability space $(\real^\pd,\bspace,\tmeas)$ where $\bspace$ are the Borel sets of $\real^\pd$ and $\tmeas$ is the distribution of $\trv$.  For this work, we will also assume that $\tmeas$ admits a corresponding density with respect to Lebesgue measure.  Let $\lebMeas$ denote the usual Lebesgue measure and let $\ntd(\trv)$ be the density associate with $\tmeas$ through:
%\[
%\tmeas(\mathcal{A}) = \int_{\mathcal{A}} \ntd(\trv)\lebMeas(d\trv)
%\]
%for any Borel set $\mathcal{A}\in\bspace$.  $\bspace$ denotes the Borel sets in $\real^\pd$.  The definition of $\tmeas$ can also be written more succinctly as the Radon-Nikodym derivative $\ntd = d \tmeas / d\lebMeas$.  Formally speaking, the quantity of interest in (\ref{eq:targetIntegral}) should be written as:
%\[
%Q = \int h(\trv)\tmeas(d\trv) =  \int h(\trv)\ntd(\trv)\lebMeas(d\trv)
%\]
%However, throughout this paper, we will only only consider continuous densities and will thus replace this Lebesgue integration with the usual Riemann integration, resulting in (\ref{eq:targetIntegral}).
%
%As mentioned above, integrals involving $\ntd$ cannot usually be evaluated analytically.  The Monte Carlo approach to overcoming this is to characterize the target density $\ntd$ with samples and then approximate the integral as a finite sum.  Assume we have $N$ samples of the target density, then (\ref{eq:targetIntegral}) can be approximated by:
%\begin{equation}
%Q \approx \frac{1}{N}\sum_{i=1}^N h(\trv^{(i)}) \label{eq:mcapprox}
%\end{equation}
%Our ultimate goal is to efficiently generate these samples.  Our approach to achieving this goal is MCMC.

%The target density cannot usually be sampled directly and only evaluations an unnormalized version of $\ntd$ are commonly available.  This is almost always the case in difficult Bayesian inference problems.   Let $\td$ (missing the normalization hat) represent a general unnormalized density satisfying
%\begin{equation}
%\ntd(\trv) = \frac{\td(\trv)}{\int \td(\trv) d\trv}
%\end{equation}
%Note that evaluating $\td$ may be computationally expensive.  Thus, our goal is to build an MCMC method that minimizes the number of required $\td$ evaluations.  This is done by reducing the correlation between states in our MCMC chain.  More details on MCMC and how such a method can be developed are given next in section \ref{sec:mcmc}.

%Throughout the forthcoming derivations and discussion, we will use several recurring variables.  These are listed in the table below for the reader's future reference.
%
%\begin{center}
%\begin{tabular}{p{0.09\textwidth}p{0.8\textwidth}}\hline
% \textbf{Symbol}	& \textbf{Description} \\\hline
% $\trv$	& Target random variable\\ 
% $\ntd$ & Normalized target density \\
%  $\td$ & Unnormalized target density\\
%  $\tilde{\td}$ & Map-induced approximation of target density $\td$ \\
%  $\tmeas$ & Target measure \\ 
%  $\qt$ & Proposal on target space\\
%  \hline
% $\rrv$	 & Reference random variable\\ 
% $\rd$ & Unnormalized reference density \\
% $\tilde{\rd}$ & Map-induced approximation of reference density $\rd$ \\
% $\rmeas$ & Reference measure \\
% $\qr$ & Proposal on reference space \\
%\hline
% $\emap$ & Exact Map from $\trv$ to $\rrv$ \\ 
%  $\imap$ & Inexact map from $\trv$ to $\rrv$ \\ 
%  %$\efspace$ & The infinite dimensional function defining $\emap$.\\
%  %$\ifspace$ & The finite dimensional function defining $\imap$. \\
%  $\mapp$ & Parameters defining the inexact transport map $\imap$ \\
%  \hline
%   $\pd$ & Dimension of sampling problem, $\trv$, and $\rrv$.\\
%   $\mathcal{B}(\mathcal{X})$ & Borel measurable sets of  $\mathcal{X}$ \\
%   $K$ & Number of samples used to approximate KL divergence \\
%   $N$ & Total number of s.pdf taken by the MCMC algorithm \\
%   $N_U$ & Number of s.pdf taken between $\imap$ adaptations in MCMC algorithm.\\
%   \hline
% \end{tabular}
%\end{center}


%---------------- OLD INTRO MATERIAL ----------------


%%% This paragraph motivates uncertainty quantification
%Scientists and engineers often rely on computer simulations to make predictions, develop understanding, and to ultimately answer questions like: \textit{what is the expected global temperature rise over the next ten years?} or \textit{how much will energy production vary in Wyoming?}  These questions can be mathematically formulated using tools from statistics and uncertainty quantification (UQ).  In the UQ setting, the answer to the above questions can be expressed as a quantity of interest, $Q$, defined by an integral over some $\pd$-dimensional random variable $\trv$ on the probability triple $(\mathcal{X},\mathcal{B}(\mathcal{X}),\tmeas)$.  Here, $\mathcal{X}\subseteq \real^\pd$ is the sample space containing all possible values of $\trv$, $\mathcal{B}(\mathcal{X})$ is the $\sigma$-algebra of Borel sets on $\mathcal{X}$, and $\tmeas$ is the distribution of $\trv$.  We assume that $\tmeas$ admits a continuous density, which allows us to write the quantity of interest as
%\begin{equation}
%Q = \int h(\trv)\ntd(\trv) d\trv.\label{eq:targetIntegral}
%\end{equation}
%Here, $\ntd(\trv)$ is the probability density related to $\tmeas$ and $h(\trv)$ is an application-specific function.  For the temperature rise example above, $\trv$ could represent current atmospheric and marine conditions, $\ntd(\trv)$ would then describe current knowledge of these conditions,  and $h(\trv)$ could be the temperature predicted by a complicated climate model using $\trv$ as initial conditions.  
%
%%% This paragraph motivates MCMC in UQ
%Unfortunately, computing expectations such as (\ref{eq:targetIntegral}) is analytically intractable in realistic situations.  A general and robust solution is then to use Monte Carlo integration to approximate (\ref{eq:targetIntegral}) with a finite set of samples $\{\trv^{(1)},\trv^{(2)},...,\trv^{(N)}\}$ taken from $\ntd(\trv)$.  The Monte-Carlo approximation is given by
%\begin{equation}
%Q \approx \frac{1}{N}\sum_{i=1}^N h(\trv^{(i)}). \label{eq:mcapprox}
%\end{equation}
%The Monte Carlo approach is easy to apply when independent samples of $\ntd(\trv)$ are efficiently obtained; however, our primary interest is in Bayesian inference problems, where the target density $\ntd(\trv)$ can be constructed from sophisticated physical models, which makes direct sampling impossible.  We therefore need more advanced methods for generating samples of $\ntd(\trv)$, such as Markov chain Monte Carlo (MCMC). 


==> Paper4Arxiv 2/mapconstruction.tex <==
\section{Construction of transport maps}
\label{sec:maps}
Transport maps will be used in Sections \ref{sec:mapmcmc} and \ref{sec:adaptmcmc} to define a new class of MCMC methods.  This section first introduces transport maps in the context of optimal transportation (Section~\ref{sec:maps:overview}) and then describes a practical method for constructing maps from samples (Section~\ref{sec:maps:construct}).


\subsection{Optimal transportation}
\label{sec:maps:overview}

Consider two Borel probability measures on $\real^{\pd}$, $\tmeas$ and $\rmeas$. We will refer to these as the \textit{target} and \textit{reference} measures, respectively, and associate them with random variables $\trv \sim \tmeas$ and $\rrv \sim \rmeas$. A transport map $\emap: \real^{\pd} \rightarrow \real^{\pd}$ is a deterministic transformation that pushes forward $\tmeas$ to $\rmeas$, yielding 
\begin{equation}
\rmeas = \emap_{\sharp} \tmeas .
\label{eq:measconst}
\end{equation}
In other words, $\rmeas(A) = \tmeas \left ( \emap^{-1}(A) \right )$ for any Borel set $A \subseteq \real^{\pd}$. In terms of the random variables, we write $\rrv \eqd \emap (\trv)$, where $\eqd$ denotes equality in distribution. The transport map induces a \textit{deterministic coupling} of probability measures \cite{Villani2009}. 

% existence and uniqueness, cost = distance squared
Of course, there can be infinitely many transport maps between two probability 
measures. On the other hand, it is possible that no transport map exists: 
consider the case where $\tmeas$ has an atom but $\rmeas$ does not. If a 
transport map exists, one way of regularizing the problem and finding a unique 
map is to introduce a cost function $c(\trv,\rrv)$ on $\real^{\pd} \times 
\real^{\pd}$ that represents the work needed to move one unit of mass from 
$\trv$ to $\rrv$. Using this cost function, the total cost of pushing $\tmeas$ 
to $\rmeas$ is
\begin{equation}
  C(\emap) = \int_{\real^{\pd}} c\left(\trv,\emap(\trv)\right) \, d \tmeas(\trv) \label{eq:mongecost}.
\end{equation}
Minimization of this cost subject to the constraint $\rmeas = \emap_{\sharp} \tmeas$ is called the Monge problem, after \cite{Monge1781}.  A transport map satisfying the measure constraint \eqref{eq:measconst} and minimizing the cost in \eqref{eq:mongecost} is an \textit{optimal} transport map. The celebrated result of \cite{Brenier1991}, later generalized by \cite{McCann1995}, shows that this map exists, is unique, and is monotone $\tmeas$-a.e.\ when $\tmeas$ is atomless and the cost function $c(\trv,\rrv)$ is quadratic. Generalizations of this result to other cost functions and spaces have been established in \cite{Champion2011, Ambrosio2013, Feyel2004, Bernard2004}.

% other couplings; Knothe-Rosenblatt as a limit of Brenier's map; nice properties of K-R.
The choice of cost function in \eqref{eq:mongecost} naturally influences the structure of the map. For illustration, consider the Gaussian case of $\trv\sim N(0,I)$ and $\rrv\sim N(0,\Sigma)$ for some positive definite covariance matrix $\Sigma$.  The associated transport map is linear: $\emap = S \trv$, where the matrix $S$ is any square root of $\Sigma$. When the transport cost is quadratic, $c(\trv,\rrv) = | \trv - \rrv |^2$, $S$ is the symmetric square root obtained from the eigendecomposition of $\Sigma$, $\Sigma = V \Lambda V^\top$ and $S = V \Lambda^{1/2} V^\top$ \cite{Olkin1982}. If the cost is instead taken to be the following weighted quadratic
\begin{equation}
  c(\trv, \rrv) = \sum_{i=1}^{\pd} t^{i-1} | \trv_i- \rrv_i |^2, \ t > 0,
  \label{eq:rosencost}
\end{equation}
then, as $t \rightarrow 0$, the optimal map becomes lower triangular and equal to
 the Cholesky factor of $\Sigma$. Generalizing to non-Gaussian 
$\tmeas$ and $\rmeas$, as $t \rightarrow 0$,  the optimal maps $\emap_t$ obtained with the cost function 
\eqref{eq:rosencost} are shown by \cite{Carlier2010} and \cite{Bonnotte2013} to 
converge to the \textit{Knothe-Rosenblatt} (KR) rearrangement 
\cite{Rosenblatt1952, Knothe1957} between probability measures. The KR map exists and is 
uniquely defined if $\tmeas$ is absolutely continuous with respect to Lebesgue 
measure.  The KR map also has several useful properties: the Jacobian matrix 
of $\emap$ is lower triangular and has positive diagonal entries $\tmeas$-a.e. 
Because of this triangular structure, the Jacobian determinant and the inverse 
of the map are easy to evaluate. This is an important computational 
advantage that we exploit in Section \ref{sec:maps:construct}.  

% We will use lower triangular structure, BUT...
We will employ lower triangular maps in our MCMC construction, but 
without directly appealing to the transport cost in \eqref{eq:rosencost}. While 
this cost is meaningful for theoretical analysis and even numerical 
continuation schemes \cite{Carlier2010}, we find that for small $t$, the sequence of weights 
$\{t^{i}\}$ quickly produces numerical underflow as the parameter 
dimension $\pd$ increases. Instead, we will directly impose the lower triangular 
structure and search for a map $\imap$ that \textit{approximately} satisfies the 
measure constraint, i.e., for which $\rmeas\approx\imap_{\sharp}\tmeas$. This 
approach is a key difference between our construction and standard optimal 
transportation. 
%We will fix the form of the map and then try to achieve the 
%coupling condition in \eqref{eq:measconst}, whereas optimal transport begins 
%with the exact coupling condition and then uses cost minimization to find a 
%map, whose form follows from the choice of transport cost. 

% 3) approximate maps: why? 
% - less complex
% - staying with approximate maps lets us impose regularity conditions that may or may not hold for the optimal map, e.g., continuous differentiability
Numerical challenges with \eqref{eq:rosencost} are not the only reason to seek approximate maps.
%; there are several other reasons, even more generally applicable. 
Suppose that the target measure $\tmeas$ is a Bayesian posterior or some other intractable distribution, but let the reference $\rmeas$ be something simpler, e.g., a Gaussian distribution with identity covariance. In this case, the complex structure of $\tmeas$ is captured by the map $\emap$. Sampling and other tasks can then be performed with the simple reference distribution instead of the more complicated distribution. In particular, if a map exactly satisfying \eqref{eq:measconst} were available, sampling the target distribution $\tmeas$ would simply require drawing a sample $\rrv^\prime \sim \rmeas$ and pushing it to the target space with $\theta^\prime = \emap^{-1}(\rrv^\prime)$. This concept was employed by \cite{Moselhy2011} for posterior sampling.
%\footnote{Note that the maps constructed in \cite{Moselhy2011} sought to push $\rmeas$ to $\tmeas$, the inverse of what is sought here.} 
 Depending on the structure of the reference and the target, however, finding an exact map may be computationally challenging. In particular, if the target contains many nonlinear dependencies that are not present in the reference distribution, the \textit{representation} of the map $\emap$ (e.g., in some canonical basis) can become quite complex.
 % (For instance, if the map is being represented as a polynomial series or with a summation of radial basis functions, many cross-terms might be required.) 
 Hence, it is desirable to work with approximations to $\emap$. Below we will demonstrate that even approximate maps can capture the key structure of the target distribution and thus be used to construct more efficient MCMC proposals.

Another reason for seeking approximate transport maps is regularity. There is an 
extensive theory on the regularity of optimal transport---with much that is 
understood, along with some open questions \cite{Caffarelli1992}. Since we are only concerned with approximate measure transformations, we can impose regularity conditions that may not hold for the optimal map or the KR map. In particular, we will require that $\imap$ and its inverse have continuous derivatives on $\real^{\pd}$, i.e., that $\imap$ be a $C^1$-diffeomorphism. Later we will impose additional constraints on the derivatives of $\imap$, which will prove useful for our theoretical analysis of map-based MCMC.


\subsection{Constructing maps from samples}\label{sec:maps:construct}

As noted above, we will seek transport maps that have a lower triangular structure, i.e.,
\begin{equation}
\emap(\trv_1,\trv_2,\ldots ,\trv_\pd) = \left[\begin{array}{l}\emap_1(\trv_1)\\ \emap_2(\trv_1,\trv_2)\\ \vdots \\ \emap_\pd(\trv_1,\trv_2,\ldots ,\trv_\pd)\end{array}\right],\label{eq:lowtriform}
\end{equation}
where $\trv_i$ denotes the $i$th component of $\trv$ and $\emap_i:\real^i 
\rightarrow \real$ is $i$th component of the map $\emap$. For simplicity, we 
assume that both the target and reference measures are absolutely 
continuous on $\real^\pd$, with densities $\pi$ and $\rd$, respectively. This 
assumption precludes the existence of atoms in $\tmeas$ and thus makes the KR 
coupling well-defined. To find a useful approximation of the KR coupling, we 
will define a map-induced density $\tilde{\td}(\trv)$ and minimize the distance 
between this map-induced density and the target density $\td(\trv)$. The next 
three subsections describe the setup of this optimization problem.

Note that when the reference measure is a standard Gaussian (as we shall prescribe below), the construction of a map from target samples to the reference is a goal shared by the iterative Gaussianization scheme of \cite{Laparra2011} and the density estimation schemes of \cite{Tabak2010,Tabak2013}. Both of these approaches \textit{compose} a series of simple maps (e.g., sigmoid-type functions of one variable in \cite{Tabak2013}) in order to achieve the desired transformation, but can require a large number of such layers in order to converge. Also, the resulting maps are not triangular. Here, we seek to develop a more expressive all-at-once approximation of the triangular KR map.%\todo{Check this paragraph.}


\subsubsection{Optimization objective}

Let $\rd$ be the probability density associated with the reference measure $\rmeas$, and consider a transformation $\imap(\trv)$ that is monotone and differentiable $\tmeas$-almost everywhere. (In Section~\ref{sec:constraints} we will discuss constraints to ensure monotonicity; moreover, we will employ maps that are everywhere differentiable by construction.) Now consider the pullback of $\rmeas$ through $\imap$. The density of this pullback measure is
\begin{equation}
\tilde{\td}(\trv) = \rd ( \imap(\trv) ) | \det \dimap(\trv) | \label{eq:mapInducedTarget},
\end{equation}
where $\demap(\trv)$ is the Jacobian of the map, evaluated at $\trv$, and $| \det \dimap(\trv) |$ is the absolute value of the Jacobian determinant. We call $\tilde{\td}$ the \textit{map-induced density}.

If the measure constraint $\rmeas = \imap_{\sharp} \tmeas$ were exactly satisfied, the map-induced density $\tilde{\td}$ would equal the target density $\td$.  This suggests finding $\imap$ by minimizing a distance or divergence; to this end, we use the Kullback-Leibler (KL) divergence,
\begin{eqnarray}
D_{\text{KL}}(\td \| \tilde{\td}) & = & \mathbb{E}_{\td}\left[\log{\left(\frac{\td(\trv)}{\tilde{\td}(\trv)}\right)}\right] \label{eq:klexpr} \\
& = & \mathbb{E}_{\td} \bigg[\log{\td(\trv)} - \log{\rd\left(\imap(\trv)\right)} - \log{\left|\det \dimap(\trv) \right|}\bigg].\nonumber
\end{eqnarray}
We can then find transport maps by solving the following optimization problem:
\begin{equation}
\min_{T \in \mathcal{T}} \mathbb{E}_{\td} \bigg[ - \log{\rd\left(\emap(\trv)\right)} - \log{\left|\det \demap(\trv) \right|}\bigg],
\label{eq:opt}
\end{equation}
% \todo{It's potentially confusing that we use $\emap$ as the dummy argument to the optimization objective above. Here it is definitely not the exact map. In fact, the optimization problem is posed to yield the approximate map. Should we replace the internal $T$ with something else?} % FIXED 
where $\mathcal{T}$ is some space of lower-triangular functions from $\real^\pd$ to $\real^\pd$. If $\mathcal{T}$ is large enough to include the KR map, then the solution of this optimization problem will exactly satisfy \eqref{eq:measconst}. Note that we have removed the $\log{\td(\trv)}$ term in \eqref{eq:klexpr} from the optimization objective \eqref{eq:opt}, as it is independent of $T$. 
If the exact coupling condition is satisfied, however, then the quantity inside the expectation in \eqref{eq:klexpr} becomes constant in $\trv$. If $\td$ is unnormalized, this constant is in fact the log of the normalizing constant of $\td$.% \cite{Moselhy2011}.

%
% YMM: Letting $\mathcal{T}$ contain all diffeomorphisms may not guarantee an exact map. Whether this function space includes K-R depends on how regular K-R is. Regularity of the Rosenblatt map: it is as regular as the densities $\rd$ and $\td$ are, but not more.

Note that the KL divergence is not symmetric.  We choose the direction above so that we can use Monte Carlo samples (in particular, MCMC samples) to approximate the expectation with respect to $\td$. Furthermore, as we will show below, this direction allows us to dramatically simplify the solution of \eqref{eq:opt} when $\rd$ is Gaussian.
%
Suppose that we have $K$ samples from $\td$, denoted by $\{\trv^{(1)},\trv^{(2)},\ldots ,\trv^{(K)}\}$. Taking a sample-average approximation (SAA) \cite{Kleywegt2002}, we replace the objective in \eqref{eq:opt} with its Monte Carlo estimate
% \begin{eqnarray}
% D_{KL}(\td \| \tilde{\td})  &\approx& \frac{1}{K}\sum_{i=1}^{K} \Bigg[\log{\td(\trv^{(k)})}  -\log{\rd\left(\emap(\trv^{(k)})\right)} - \log{\left|\det \demap(\trv^{(k)}) \right|}\Bigg]\label{eq:mckl}.
% \end{eqnarray}
and, for this fixed set of samples, solve the corresponding deterministic optimization problem:
\begin{equation}
\imap = \arg \min_{T \in\mathcal{T}} \frac{1}{K}\sum_{k=1}^{K} \Bigg[ -\log{\rd\left(\emap(\trv^{(k)})\right)} - \log{\left|\det \demap(\trv^{(k)}) \right|}\Bigg].
\label{eq:mckl}
\end{equation}
The solution $\imap$ is an approximation to the exact transport map for two reasons: first, we have used an approximation of the expectation operator; and second, we have restricted the feasible domain of the optimization problem to $\mathcal{T}$. The specification of $\mathcal{T}$ is the result of constraints, discussed in Section~\ref{sec:constraints}, and of the finite-dimensional parameterization of the map, discussed in Section~\ref{sec:maps:param}. 


% OMITTED BELOW: this is true and good to point out, but it requires that the optimization problem have a unique minimum. So let's delay it until we show that the optimization problem is strictly convex!
% 
% Of course, as the feasible domain is enriched and $K \rightarrow \infty$, $\imap$ should approach the exact Knothe-Rosenblatt map.




%%%%%%%%%%%%%%%%%%
% QUESTIONS AND TODO 11/18:

% What conditions on T are required to write the density of the pullback as in (5)? Differentiable, certainly. But monotone? Note that monotonicity implies a.e. differentiability on \real. Does it imply this on \real^n too? If not, then do we need to require differentiability explicitly? Go further and require bijection and diffeomorphism (cont diff and cont diff inverse)?

% Could we recast these conditions as the Jacobian existing and being positive definite a.e. (for strictly monotone)? Positive semi-definite (for monotone)? What do we really need here? Answer: NO, all true but kind of a digression!

% Does being bi-Lipschitz imply the derivative constraint? Yes.

% But is it true other way around? Does differentiability with a lower bound on the derivative imply the lower Lipschitz condition? Not totally clear; see Florian's email.

% Will we keep map parameters (e.g., polynomial coeffs) in a compact space? (Answer: sure, but not a big deal.)

% Look at Rosenblatt and Knothe papers for fine properties of the KR map.

\subsubsection{Constraints}
\label{sec:constraints}
To write the map-induced density $\tilde{\td}$ as in 
\eqref{eq:mapInducedTarget}, it is sufficient that $\imap$ be differentiable and 
monotone, i.e., $( \trv^\prime - \trv) ^\top ( \imap(\trv^\prime) - 
\imap(\trv)  )\geq 0$ for distinct points $\trv, \trv^\prime \in \real^\pd$. 
Since we assume that $\tmeas$ has no atoms, to ensure that the pushforward 
$\imap_\sharp \tmeas$ also has no atoms we only need to require that $\imap$ be strictly monotone.
%
% In particular, we need the Jacobian of $\imap$ to be positive definite on the support of $\td$, i.e.,
% \begin{equation}
% \dimap(\trv) \succ 0 \quad \forall \trv \in \supp{\pi} \label{eq:positivityeverywhere}.
% \end{equation}
% This condition implies that the determinant $\det \dimap(\trv) $ is also positive on $\supp(\td)$. 
%
To show ergodicity of the MCMC samplers constructed in Sections~\ref{sec:mapmcmc} and \ref{sec:adaptmcmc}, however, we will need to impose the stricter condition that $\imap$ be bi-Lipschitz,
\begin{eqnarray}
 \lambda_{\text{min}}  \|\trv^\prime - \trv \| \leq \|\imap(\trv^\prime) - \imap(\trv)\| \leq  \lambda_{\text{max}} \|\trv^\prime - \trv \| \label{eq:dUB},
\end{eqnarray}
for some $0 < \lambda_{\text{min}} \leq \lambda_{\text{max}} < \infty$. This condition implies that $\imap$ is differentiable almost everywhere. But the maps we will employ are, by construction, everywhere differentiable and lower triangular, and hence the lower Lipschitz condition in \eqref{eq:dUB} is equivalent to a lower bound on the map derivative,
%\todo{This is related to Florian's note.}
\begin{equation}
\frac{\partial \imap_i}{ \partial \trv_i} \geq \lambda_{\text{min}} \label{eq:derivLB}, \ i=1 \ldots \pd. 
\end{equation}
Since $\imap$ is lower triangular, the Jacobian $\dimap$ is also lower triangular, and \eqref{eq:derivLB} ensures that the Jacobian is positive definite. Because the Jacobian determinant is then positive, we can remove the absolute value from the determinant terms in \eqref{eq:opt}, \eqref{eq:mckl}, and related expressions. This is an important step towards arriving at a convex optimization problem (see Section~\ref{subsubsec:convex}).  We stress that while a nonzero $\lambda_{\text{min}}$ is required for our theoretical analysis, it does not need to be tuned in order to apply the algorithm in practice; typically we just choose a very small value, e.g.,  $\lambda_{\text{min}} = 10^{-8}$.  An explicit value for $\lambda_{\text{max}}$ can also be prescribed, but can instead be defined implicitly through the construction described next.

Many representations of $\imap$ (e.g., polynomial expansions) will yield maps with unbounded derivatives as $\|\trv\|\rightarrow \infty$.  Clearly, such maps would not satisfy the upper bound in \eqref{eq:dUB}.  Fortunately, a simple correction ensures \eqref{eq:dUB} is satisfied. 
%
Let $\imap: \real^\pd \rightarrow \real^\pd$ be a continuously differentiable function whose derivatives grow without bound as $\|\trv\|\rightarrow \infty$, but are finite within a ball $B(0,R)$ of radius $R<\infty$.  We can satisfy \eqref{eq:dUB} by setting $\imap^R(\trv) = \imap(\trv)$ over $B(0,R)$ and forcing $\imap^R(\trv)$ to be linear outside of this ball.  More precisely, let $w(\trv) := R\frac{\trv}{\|\trv\|}$ be the projection of $\trv$ to the closest point in $B(0,R)$ and let $d(\trv): = \frac{\trv}{\|\trv\|}\cdot \nabla \imap(w(\trv))$ be the directional derivative of $\imap$ at the ball boundary. We then define $\imap^R(\trv)$ in terms of $\imap(\trv)$ as
\begin{equation}
\imap^R(\trv) = \left\{ \begin{array}{ll} \imap(\trv) & \quad \|\trv\|\leq R\\ \imap\left(w(\trv)\right) + d(\trv)(\trv-w(\trv)) &  \quad \|\trv\|> R \end{array}\right. .\label{eq:ubMap}
\end{equation}
Note that a continuously differentiable $\imap(\trv)$ will yield a continuously differentiable $\imap^R(\trv)$. Moreover, if $\imap(\trv)$ satisfies the lower bound in \eqref{eq:dUB}, $\imap^R(\trv)$ will satisfy both the lower and upper bounds in \eqref{eq:dUB}. 

% \begin{figure}[h]
% \centering
% \input{pics/mcmc/DerivativeBoundedPoly.tex}
% \caption[Ensuring bounded map derivatives with linear correction.]{Illustration of the difference between $\imap(\trv)$ and $\imap^R(\trv)$ in \eqref{eq:ubMap}.  In this one dimensional illustration, $\imap(\trv)$ and $\imap^R(\trv)$ are identical for $\trv\in[-R,R]$; however, when $\trv$ is outside this interval, $\imap^R$ becomes linear.  The slope of $\imap^R(\trv)$ for $\trv>R$ is given by $d\imap/d\trv$ evaluated at $R$.}
% \label{fig:ubMap}
% \end{figure}

When a finite number of samples are used in the Monte Carlo sum of \eqref{eq:mckl}, $R$ can usually be chosen so that all the samples lie in $B(0,R)$, and hence $\imap$ can be evaluated directly.  In this setting, a value of $R$ need not be explicitly prescribed. However, our asymptotic convergence theory requires finite derivatives of the map as $\|\trv\|\rightarrow \infty$ in order to achieve the correct tail behavior, which is guaranteed by using $\imap^R$ as in \eqref{eq:ubMap}.

Unfortunately, we cannot generally enforce the lower bound in \eqref{eq:derivLB} over the entire support of the target measure.  A weaker, but practically enforceable, alternative is to require the map to be increasing at each sample used to approximate the KL divergence. In other words, we use the constraints
\begin{equation}
\left.\frac{\partial \imap_i}{\partial \trv_i}\right|_{\trv^{(k)}} \geq \lambda_{\text{min}} \quad \forall  i \in\{1,2,\ldots, \pd \}, \ \forall k \in\{1,2,\ldots, K\}\label{eq:mono2}.
\end{equation}
Practically, we have found that \eqref{eq:mono2} is sufficient to ensure the monotonicity of a map represented by a finite basis expansion.

\subsubsection{Convexity and separability of the optimization problem}
\label{subsubsec:convex}

Now we consider the task of minimizing the objective in \eqref{eq:mckl}.  The $1/K$ term can immediately be discarded, and the derivative constraints above let us remove the absolute value from the determinant term. % The optimization problem then becomes
% \begin{align}
% \min_{T \in\mathcal{T}} \sum_{k=1}^{K} \Bigg[ -\log{\rd\left(\emap(\trv^{(k)})\right)} - \log{ \det \demap(\trv^{(k)}) }\Bigg]
% \label{eq:klcost}.
% \end{align}
While one could tackle the resulting minimization problem directly, we can simplify it further by exploiting the structure of the reference density and the triangular map.

First, we let $\rrv\sim N(0,I)$.  This choice of reference distribution yields
\begin{equation}
\log\rd(\rrv) = -\frac{\pd}{2}\log(2\pi) - \frac12\sum_{i=1}^\pd\rrv_i^2. \label{eq:gaussPart}
\end{equation}
Next, the lower triangular Jacobian $\dimap$ simplifies the determinant term in \eqref{eq:mckl} to give
%recall that the Jacobian matrix $\dimap$ is lower triangular.  This allows the determinant term in \eqref{eq:mckl} to be written as
\begin{equation}
\log{\left|\det \dimap(\trv) \right|} = 
\log{ ( \det\dimap(\trv) )} = \log\left(\prod_{i=1}^{\pd} \frac{\partial \imap_i}{\partial \trv_i}\right) = \sum_{i=1}^{\pd}\log\frac{\partial \imap_i}{\partial \trv_i} \label{eq:detexp}.
\end{equation}
The objective function in \eqref{eq:mckl} now becomes
\begin{equation}
C(\imap) = \sum_{i=1}^{\pd} \sum_{k=1}^{K}\left[  \frac12 \imap_i^2(\trv^{(k)}) - \log\left.\frac{\partial \imap_i}{\partial \trv_i}\right|_{\trv^{(k)}}\right]\label{eq:fullopt}.
\end{equation}
This objective is \textit{separable}: it is a sum of $\pd$ terms, each involving a single component $\imap_i$ of the map. The constraints in \eqref{eq:mono2} are also separable; there are $K$ constraints for each $\imap_i$, and no constraint involves multiple components of the map. Hence the entire optimization problem separates into $\pd$ individual optimization problems, one for each dimension of the parameter space. Moreover, each optimization problem is \textit{convex}: the objective is convex and the feasible domain is closed (note the $\geq$ operator in the linear constraints \eqref{eq:mono2}) and convex.

% By closing the set of feasible maps (i.e., \eqref{eq:derivLB} has a $\geq$ while \eqref{eq:positivityeverywhere} uses a $>$), we have made the feasible domain of this optimization problem convex.  Because the objective is also convex, we have a convex optimization problem that can be solved efficiently. 


% \subsubsection{Separating the optimization problem}
% \label{sec:maps:sepopt}

In practice, we must solve the optimization problem over some finite-dimensional space of candidate maps. Let each component of the map be written as $\imap_i(\trv;\mapp_i)$, $i=1\ldots \pd$, where $\mapp_i \in \real^{M_i}$ is a vector of parameters, e.g., coordinates in some basis. 
%Throughout this work, we employ multivariate Hermite polynomial basis functions (see supplementary material for details), but other choices are certainly possible.  For instance, \cite{Parno2014thesis} found radial basis function representations of the map also to be useful. For any choice of basis, we will require that $\imap_i$ be linear in $\mapp_i$. 
The complete map is then defined by the parameters $\mappa = [\mapp_1, \mapp_2,\ldots , \mapp_{\pd}]$. Note that there are distinct parameter vectors for each component of the map. The optimization problem over the parameters remains separable, with each of the $\pd$ different subproblems given by:
\begin{equation}
\begin{aligned}
& \underset{\mapp_i}{\min}
& & \sum_{k=1}^{K}\left[  \frac12 \imap^2_i(\trv^{(k)}; \mapp_i) - \log\left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}}\right]\\
& \text{s.t.}
& & \left.\frac{\partial \imap_i(\trv;\mapp_i)}{\partial \trv_i}\right|_{\trv^{(k)}} \geq \lambda_{\text{min}}, \quad k\in\{1,2,\ldots ,K\},
\end{aligned}\label{eq:basicopt}
\end{equation}
for $i=1\ldots \pd$. All of these optimization subproblems can be solved in parallel without evaluating the target density $\td(\trv)$. Since the map components $\imap_i$ are linear in the coefficients $\mapp_i$, each finite-dimensional problem is still convex.  
%Moreover, efficient matrix-matrix and matrix-vector operations can be used to evaluate the objective.  This allows us to easily solve (\ref{eq:basicopt}) with a standard Newton method. 

\subsection{Map parameterization}
\label{sec:maps:param}
In this work, we parameterize each component of the map $\imap_i$ with a multivariate polynomial expansion.  Each multivariate polynomial $\psi_{\mathbf{j}}$ is defined as
\begin{equation}
\psi_{\mathbf{j}}(\trv) = \prod_{i=1}^{\pd} \varphi_{j_i}(\trv_i).
\end{equation}
where $\mathbf{j} = (j_1,j_2, \ldots , j_{\pd} ) \in \mathbb{N}_0^{\pd}$ is a multi-index and $\varphi_{j_i}$ is a univariate polynomial of degree $j_i$. The univariate polynomials can be chosen from any family of orthogonal polynomials (e.g., Hermite, Legendre, Jacobi); even monomials are sufficient for the present purposes.\footnote{In principle, there is some advantage to choosing polynomials that are orthogonal with respect to the input distribution $\tmeas$, as in polynomial chaos approaches \cite{GhanemBook,LeMaitre2010}.
% for instance, moments of $\tmeas$ could then be estimated from the polynomial coefficients of a sufficiently accurate map. 
In the present context, however, we only have samples from $\tmeas$, and this distribution is almost certainly not one of the canonical distributions found in the Wiener-Askey scheme \cite{Xiu2002}. Thus $\tmeas$-orthogonal polynomials are not readily available, and there is little reason to be picky about the choice of polynomial basis.}
%
Using these multivariate polynomials, we express the map as a finite expansion of the form
\begin{equation}
\imap_i(\trv; \mapp_i) = \sum_{\mathbf{j}\in\mathcal{J}_i} \mapp_{i,\mathbf{j}} \, \psi_{\mathbf{j}}(\trv) \label{eq:polyexpand},
\end{equation}
where $\mathcal{J}_i$ is a set of multi-indices defining the polynomial terms in the expansion.  Notice that the cardinality of the multi-index set defines the dimension of each parameter vector $\mapp_i$, i.e., $M_i = |\mathcal{J}_i|$.  An appropriate choice of each multi-index set $\mathcal{J}_i$ will force the entire map $\imap$ to be lower triangular.  
%This paper's supplementary material gives examples of this construction and more information on choosing appropriate multi-index sets.

One simple choice of the multi-index set corresponds to a total-order polynomial basis, where the maximum degree of each multivariate polynomial is bounded by some integer $p \geq 0$:
\[
\mathcal{J}^{TO}_{i} = \{ \mathbf{j} : \| \mathbf{j}\|_1 \leq p, \ j_k=0 \ \forall k > i \}.
\]
The first constraint in this set limits the polynomial order, while the second 
constraint, $j_k=0 \ \forall k > i$, applied over all $i=1\ldots \pd$ components 
of the map, forces $\imap$ to be lower triangular.  
% However, the number of  terms in $\mathcal{J}_{i}^{TO}$ can grow quite rapidly with $i$ and $p$.
A  smaller multi-index set for large $\pd$ can be obtained by removing all the 
mixed terms in the basis:
\[
  \mathcal{J}^{NM}_{i} = \{ \mathbf{j} : \|\mathbf{j}\|_1 \leq p, \  j_k j_m=0 \ \forall k \neq m,  \  j_k=0 \ \forall  k > i \}.
\] 
An even more parsimonious option is to use diagonal maps, via the multi-index sets
\[
  \mathcal{J}^{D}_{i} = \{ \mathbf{j} : \|\mathbf{j}\|_1 \leq p, \ j_k=0 \  \forall k \neq  i\}.
\] 
We will occasionally use a union of low degree $\mathcal{J}^{TO}_{i}$ and high degree $\mathcal{J}^{D}_{i}$ to define expressive map expansions with a tractable number of terms.
%Figure \ref{fig:multindexSets} illustrates the difference between these three sets for $p=3$ and $\pd = 2$.  As the parameter dimension increases, it becomes more important to choose a basis set that balances the map's expressive power with its computational cost.

%\todo{The distinction between ``no mixed terms'' and ``no cross terms'' is not very obvious just from the labels. How about total order, no mixed = no cross, and diagonal. The text above now avoids this ambiguity, but I think we should revise the superscripts on $\mathcal{J}$ and the legend in the figure below accordingly.}

%\todo{Also, what about truncating the figure at $j_1= j_2 = 4$ rather than $5$, to save space?}

%\begin{figure}[h]
%\centering 
%
%
%\iftoggle{enableTikz}{
%\begin{tikzpicture}
%
%\node[anchor=south] at (2,4.6) {Terms in multi-index set};
%
%\foreach \i in {-0.5,0.5,...,4.5} {
%        \draw [very thin,gray] (\i,-0.5) -- (\i,4.5);
%    }
%    \foreach \i in {0,1,...,4} {
%        \node[anchor=north] at (\i,-0.55) {$\i$};
%    }
%    \foreach \i in {-0.5,0.5,...,4.5} {
%        \draw [very thin,gray] (-0.5,\i) -- (4.5,\i);
%    }
%   \foreach \i in {0,1,...,4} {
%        \node[anchor=east] at (-0.55,\i) {$\i$};
%    }
%    
%    \node[anchor=north] at (2,-1) {$j_1$};
%  \node[anchor=east] at (-1,2) {$j_2$};
%  
%      \foreach \i in {0,...,3}{
%        \foreach \j in {0,...,\i}{
%          \draw[fill=green!70!black] (3-\i,\j) circle (0.45);
%        }
%      }
%    \foreach \i in {0,...,3}{
%        \draw[fill=blue] (0,3-\i) circle (0.3);
%      }
%    \foreach \i in {0,...,3}{
%        \draw[fill=red!70!black] (3-\i,0) circle (0.15);
%        \draw[fill=red!70!black] (0,3-\i) circle (0.15);
%      }
%
%\node[anchor=west] at (5,3) {\tikz{ \draw[fill=green!70!black] circle (0.7ex); } Total order set $\mathcal{J}^{TO}_{2}$.};
%\node[anchor=west] at (5,2) {\tikz{ \draw[fill=blue] circle (0.7ex); } Set of diagonal terms $\mathcal{J}^{D}_{2}$.};
%\node[anchor=west] at (5,1) {\tikz{ \draw[fill=red!70!black] circle (0.7ex); } Set with no mixed terms $\mathcal{J}^{NM}_{2}$.};
%\end{tikzpicture}
%}{
%\includegraphics{pics/tikz-external/arxiv_main-figure1.pdf}
%}
%
%\caption[Visualization of multi-index sets.]{Visualization of multi-index sets for the second component of a two-dimensional map, $\imap_2(\trv_1,\trv_2)$.  In this case, $j_1$ is the degree of a univariate polynomial in $\trv_1$ and $j_2$ is the degree in $\trv_2$.  A filled circle indicates that a term is present in the set of multi-indices.}
%\label{fig:multindexSets}
%\end{figure}

Finally, we emphasize that \textit{any} parameterization of the map that is linear in the coefficients $\mappa$ can be used in the optimization problems defined earlier. While the examples in this paper will focus on polynomial maps, we have also had good success representing the map as a summation of linear terms and radial basis functions \cite{Parno2014thesis}.


\subsection{Solving the map optimization problem}\label{sec:maps:efficient}
Since the map $\imap_i(\trv; \mapp_i)$ is linear in the expansion coefficients $\mapp_i$, the objective in \eqref{eq:fullopt} can be evaluated using efficient matrix-matrix and matrix-vector operations.  We first construct matrices $F_i, G_i\in \real^{K\times M_i}$ with components defined by $[F_{i}]_{k, \mathbf{j}} = \psi_{\mathbf{j}}(\trv^{(k)})$ and $[G_{i}]_{k, \mathbf{j}}  = \left . \frac{\partial \psi_{\mathbf{j}}}{\partial \trv_i}  \right |_{\trv^{(k)}}$ for all $\mathbf{j}\in \mathcal{J}_i$.  Recall that $K$ is the number of samples in our Monte Carlo approximation of the optimization objective.  Using these matrices and the expansion \eqref{eq:polyexpand}, we can rewrite \eqref{eq:fullopt} as
\begin{equation}
\begin{aligned}
& \underset{\mapp_i}{\min}
& & \frac{1}{2} \mapp_i^\top(F_i^\top F_i)\mapp_i - c^\top\log(G_i\mapp_i)\\
& \text{s.t.}
& & G_i\mapp_i \geq \lambda_{\text{min}}, 
\end{aligned}\label{eq:basicopt2}
\end{equation}
where $c$ is a $K$-dimensional vector of ones and the $\log$ is taken componentwise.  Clearly, the objective can be evaluated with efficient numerical linear algebra routines.
 
% \begin{figure}[h]
%\centering
%
%\iftoggle{enableTikz}{
%
%\begin{tikzpicture}
%\node[anchor=south west, inner sep=0] (image) at (0,0) {\includegraphics[width=0.45\textwidth]{pics/mcmc/ObjectiveLandscape.pdf}};
%\begin{scope}[x={(image.south east)},y={(image.north west)}]
%        \draw[->,black,ultra thick,rounded corners] (0,0) -- (1.01,0);
%         \draw[->,black,ultra thick,rounded corners] (0,0) -- (0.0,1.01);
%         \node[anchor=north, inner sep=0] at (0.5,-0.02) {Map slope};
%         \node[rotate = 90, anchor=south, inner sep=0] at (-0.02,0.5) {Map intercept};
%         \node (optText) at (0.7,0.5) {Optimal coefficients};
%         \node (optPt) at (0.49,0.37) {};
%         \draw[->] (optText) -- (optPt);
% \end{scope}
% \end{tikzpicture}
% }{
% \includegraphics{pics/tikz-external/arxiv_main-figure2.pdf}
% }
% 
%
%
%\caption[Typical objective function in map construction.]{Illustration of the objective function in (16*) for a Gaussian $\td$ and linear map.  The color map represents values of the objective in \eqref{eq:basicopt2}.  The lightly shaded region to the left of the black contour is the region of the parameter space where the $\log$ term is larger than the quadratic term in the objective.  Clearly the problem is convex and most of the solution space is dominated by the quadratic term.  These features make Newton methods particular efficient for solving this problem.}
%\label{fig:objectiveLandscape}
%\end{figure}

Beyond efficient evaluations, the only difference between \eqref{eq:basicopt2} and a simple quadratic program is the log term in the objective.  However, the quadratic term often dominates the log term, making a standard Newton optimizer with backtracking line search quite efficient.  In practice, starting with an identity map, we usually observe convergence in fewer than ten Newton iterations.
Notice also that the log term in \eqref{eq:basicopt2} acts as a barrier function for the constraints.
% We should also point out that the constraints are never active at the solution of this problem because the log term in \eqref{eq:basicopt2} acts as a barrier function for the constraints.


==> Paper4Arxiv 2/mcmc.tex <==
\section{Map-based MCMC proposals}
\label{sec:mapmcmc}
% \todo{revision notes in TeX}
%
% abridge the opening; lots of redundant or unnecessary info here
% key idea: 
% --> this section will show how to modify MCMC *given* an approximate transport map \imap
% --> next section will show how to iteratively build such a map, in an adaptive MCMC framework

Now we will show how a transport map can be used to modify the Metropolis-Hastings algorithm by equivalently transforming either the target distribution or the proposal mechanism. In this section, we assume that a {fixed} transport map $\imap$ is in hand. Of course, this map must somehow be constructed, and hence the fixed-map approach described here is just an intermediate step in our exposition. The next section (Section~\ref{sec:adaptmcmc}) will use the optimization approaches of Section~\ref{sec:maps} to iteratively build such a map in an adaptive MCMC framework.

A simple Metropolis-Hastings algorithm \cite{Hastings1970,Metropolis1953} generates a new state $\trv^{(k+1)}$ from the current state $\trv^{(k)}$ in two s.pdf.  First, a sample $\trv'$ is drawn from a proposal density $q_{\trv,\bar{\mapp}}( \cdot |\trv^{(k)})$.  Then, an accept-reject step is performed: $\trv^{(k+1)}$ is set to $\trv^\prime$ with probability $\alpha(\trv^\prime,\trv^{(k)})$ and to $\trv^{(k)}$ with probability $1-\alpha(\trv^\prime,\trv^{(k)})$, where
\begin{equation}
\alpha\left(\trv^\prime,\trv^{(k)}\right) = 
\min\left\{1,\frac{\td(\trv^\prime)q_{\theta,\bar{\mapp}}(\trv^{(k)} | 
\trv^\prime)}{\td(\trv^{(k)})q_{\theta,\bar{\mapp}}(\trv^\prime | \trv^{(k)})} 
\right\}\label{eq:basicmh}.
\end{equation}  
The choice of proposal $q_{\trv,\bar{\mapp}}$ controls the dependence between successive states in the MCMC chain through both the acceptance rate and the step size. Knowledge of the target density $\td$ is helpful in designing proposals to make large moves that simultaneously have a high acceptance probability. The scheme presented here encodes information about the target distribution via a transport map $\imap$.

% Since the correlation in the Markov chain can dramatically alter the accuracy of a Monte Carlo approximate based on the samples, it is important to to use a proposal distribution that proposes large s.pdf with a high probability of acceptance.  Appropriately tuning proposal parameters is required to make almost any classic proposal mechanis efficient.  Examples include the variance of a Random-Walk Metropolis (RWM) proposal, the step size of a Metropolis-Adjusted Langevin Algorithm (MALA) proposal, or the number of steps in a Harmiltonian Monte Carlo (HMC) proposal.  While theoretical results such as those found in \cite{Roberts2001} provide guidelines for optimally tuning proposal parameters, hand tuning these parameters can be a difficult and time-consuming task.  Adaptive strategies try to overcome this issue by learning the proposal parameters as the MCMC chain progresses.  
 
% In the RWM and MALA proposals, the previous states can be used to obtain sample estimates of the target covariance.  The proposal covariance can then be set to a scaled version of sample covariance.  In the RWM case, this idea leads to the ``Adaptive Metropolis" (AM) algorithm first proposed in \cite{Haario2001}.  For the MALA case, this type of covariance adaptation is discussed in \cite{Atchade2006}.  By matching the proposal covariance to the target covariance, the proposals can take much larger s.pdf and still stay within high density regions of the parameter space.  
 
% % SAVE FOR LATER
% While a chain constructed with an adaptive proposal is not strictly Markov, the adaptive chain can still be ergodic under some surprisingly mild conditions on the sequence of proposal distributions $\qt^{(k)}$ \cite{Andrieu2006}.  More on the convergence properties of adaptive MCMC will be discussed in Section \ref{sec:convergence}, where we show the ergodicity of our own adaptive approach.

% \subsection{Combining maps and MCMC}

% Assume for this section that we have a previously constructed approximate map $\imap(\trv)$.  Unfortunately, using an approximate map to sample the target density $\td(\trv)$ directly will yield \textit{inexact} samples.  However, the map can still capture much of the target distribution's structure and we can exploit that by combining the map with either a local or independent Metropolis-Hastrings proposal distribution on the reference space.  Combining the approximate map with the reference proposal $q_\rrv(\rrv' | \rrv)$ will create an efficient map-induced target proposal denoted by $q_{\trv,\bar{\mapp}}(\trv^\prime | \trv)$.  When the map is fixed, this process can be viewed in two ways: (1) the canonical reference proposal  $q_r(\rrv' | \rrv)$ is applied to a map-induced approximate reference density $\tilde{\rd}(\rrv)$, or (2) the map-induced target proposal $q_{\trv,\bar{\mapp}}(\trv^\prime | \trv)$ is applied to the original target density $\td(\trv)$.  The details below will generally follow this second map-induced proposal view, but readers may find the first idea of transforming or ``preconditioning'' the target density intuitively useful.

\subsection{MCMC with a fixed transport map}
\label{sec:mapmcmc:proposal}
Assume that we have an approximate transport map $\imap$ between a standard Gaussian reference and the target measure $\tmeas$, i.e., $\rmeas\approx\imap_{\sharp}\tmeas$. The pushforward of the target measure through this map will not be Gaussian. But a map that reduces the optimization objective of Section~\ref{sec:maps} will make the pushforward closer  (in this particular sense) to a standard Gaussian than the original target. We will then use MCMC to sample this pushforward distribution, with a proposal $q_r(\rrv' | \rrv)$. The proposal $q_r$ may be chosen quite freely, and examples below will encompass both local and independence proposals. Equivalently, one can view this process from the perspective of the target space by considering the pullback through the map $\imap$ of the proposal $q_r$; this map-induced proposal is applied to the original target density $\td$. Below we will describe our algorithm from this second perspective, but the first perspective of  transforming or ``preconditioning'' the target density may also provide useful intuition.

Let  $q_r(\rrv^\prime | \rrv)$ be a standard Metropolis-Hastings proposal on the reference space. The pullback of this proposal through $\imap$ induces a target-space proposal density written as
\begin{equation}
q_{\trv,\bar{\mapp}}(\trv^\prime | \trv) = q_\rrv \left ( \imap(\trv^\prime) | \imap(\trv)\right) \left | \det \dimap(\trv^\prime) \right | , \label{eq:mapprop}
\end{equation}
where $\bar{\mapp}$ denotes the dependency of this proposal on the map parameters.  To perform MCMC, we need the ability to evaluate this proposal density and to draw samples from it.  The expression \eqref{eq:mapprop} provides an easy way of evaluating the proposal density. Sampling from the proposal $q_{\trv,\bar{\mapp}}( \cdot | \trv)$ involves three s.pdf: (1) use the current target state $\trv$ to compute the current reference state, $r=\imap(\trv)$; (2) draw a sample $\rrv^\prime \sim q_\rrv(\rrv^\prime | \rrv)$ from the reference proposal; and (3) evaluate the inverse map at $\rrv^\prime$ to obtain a sample from the target proposal: $\theta^\prime = \imap^{-1}(\rrv^\prime)$. These steps are given as lines 4--6 of Algorithm \ref{alg:adaptalg} and illustrated in Figure \ref{fig:propProcess}. Ignoring the adaptation in lines 9--13, Algorithm \ref{alg:adaptalg} is equivalent to a standard Metropolis-Hastings algorithm on the target distribution, using $q_{\trv,\bar{\mapp}}(\trv^\prime | \trv)$ as a proposal.

% Using this proposal process in a standard Metropolis-Hastings algorithm yields the method in Algorithm \ref{alg:fixedalg}.

Because of the map's lower triangular structure, evaluating the inverse map $\imap^{-1}(\rrv)$ only requires $\pd$ one-dimensional nonlinear solves. These one-dimensional problems can be tackled efficiently with a simple Newton method or, if the map is represented with polynomials, with a bisection solver based on Sturm sequences \cite{Wilf1978}.  We utilize the latter approach because of its robustness.  

% include a figure illustrating the sampling procedure
\input{pics/mcmc/SamplingProcess.tex}


% \begin{algorithm}
% % YMM: all the subscript c notation seemed strange, so I got rid of it... 
% \DontPrintSemicolon
% \KwIn{Initial state $\trv_0$, preconstructed transport map $\imap(\trv)$, valid reference proposal $q_r( r' | r^{(k)} )$}
% \KwOut{MCMC samples of the target distribution $\left\{\trv^{(1)},\trv^{(2)},\ldots,\trv^{(K)}\right\}$}
% Set $\trv^{(1)} = \trv_0$\\
% \For{$k \gets 1$ \textbf{to} $K-1$}{
% Compute the reference state, $\rrv^{(k)} = \imap(\trv^{(k)})$\;
% Draw a sample from the reference proposal, $\rrv^\prime\sim q_\rrv( \cdot |\rrv^{(k)})$\;
% Compute the target proposal sample, $\trv^\prime = \imap^{-1}(\rrv^\prime)$\;
% Calculate the acceptance probability:
% \begin{equation*}
% \alpha = \min\left\{1, \frac{\td( \trv^\prime) }{\td( \trv^{(k)} ) } \frac{q_r\left(\rrv^{(k)}|\rrv^\prime\right)}{q_r\left(\rrv^\prime|\rrv^{(k)}\right)}\frac{\det | D \imap^{-1}(\rrv^\prime) |}{\det | D \imap^{-1}(\rrv^{(k)}) |}\right\}\label{eq:fixedaccept}
% \end{equation*}\;
% Set $\trv^{(k+1)}$ to $\trv^\prime$ with probability $\alpha$; else set $\trv^{(k+1)} = \trv^{(k)}$.\;
% }
% \Return{Target samples $\left\{\trv^{(1)},\trv^{(2)},\ldots,\trv^{(K)}\right\}$}
% \caption{MCMC algorithm with fixed map}
% \label{alg:fixedalg}
% \end{algorithm}
%\todo{Above we should decide whether to keep $\rrv$ as is or to call it $\rrv^{(k)}$ for consistency with $\trv$.}
%\todo{Double-check which determinant term in the acceptance probability above has $\rrv$ or $\rrv'$!}

\subsection{Derivative-based proposals}
\label{sec:mapmcmc:deriv}
An important feature of our approach is that the map-induced proposal $q_{\trv,\bar{\mapp}}(\trv^\prime | \trv)$ requires derivative information from the target density $\td(\trv)$ if and only if the reference proposal $q_\rrv(\rrv^\prime | \rrv)$ explicitly requires derivative information.  
%In other words, if $q_r$ requires only density evaluations, then our method will only require evaluations of $\td$. On the other hand, if simulating and evaluating $q_r$ requires the gradient of the target density (as in a Langevin proposal, for example), then we must compute gradients of the pushforward of the target density to the reference space.
%
We also note that Algorithm \ref{alg:adaptalg} does not require $\td(\trv)$ to take any particular form (e.g., to be a Bayesian posterior or to result from a Gaussian prior). The ability to work with arbitrary target distributions for which derivative information may not be available is a distinction from many recent sampling approaches, such as Riemannian manifold MCMC \cite{Girolami2011}, the No-U-Turn Sampler of \cite{Hoffman2011}, or optimization-based samplers such as implicit sampling or RTO \cite{Morzfeld2012,Bardsley2014}.  
%
That said, though our approach can perform quite well without derivative information, we can still accommodate proposals that employ it.  

% If q_r is the proposal of a Langevin scheme, it will require gradients of the density of the pushforward of the target to the reference space.

%Here we show that a simple application of the chain rule allows us propagate target density derivatives through the transport map, which then enables us to use reference proposals that exploit derivative information.  

The reference proposal $q_\rrv$ is applied to the pushforward distribution of the target $\pi$ through the map $\imap$. Let  $\tilde{\rd}$ denote the corresponding pushforward density. %   with density denoted by $\tilde{\rd}$.
% with density given by:
%\begin{equation}
%\tilde{\rd}(\rrv) = \td \left ( \imap^{-1}(\rrv) \right)  | \det D \widetilde{T}^{-1}(\rrv) | \label{eq:referenceTarget}.
%\end{equation}
Taking advantage of the map's lower triangular structure,  we can write the logarithm of this density as
\begin{equation}
\log\tilde{\rd}(\rrv) = \log\td \left (\imap^{-1}(\rrv) \right ) + \sum_{i=1}^\pd\log\frac{\partial \widetilde{T}_i^{-1}}{\partial \rrv_i} \label{eq:referenceTarget}.
\end{equation}
We will use the chain rule to obtain the gradient of this expression.  First, make the substitution $\rrv=\imap(\trv)$ and take the gradient with respect to $\trv$:
\begin{equation}
\nabla_\trv \log\tilde{\rd} \left (\imap(\trv) \right ) =  \nabla_\trv\log\td(\trv) -\sum_{i=1}^\pd \left(\frac{\partial \imap_i}{\partial \trv_i}\right)^{-1} H_i(\trv),
\end{equation}
where $H_i$ is a row vector of second derivatives coming from the determinant term: $H_i(\trv) = \left[\begin{array}{cccc}\frac{\partial^2 \imap_i}{\partial \trv_1 \partial \trv_i} & \frac{\partial^2 \imap_i}{\partial \trv_2 \partial \trv_i}  & \cdots & \frac{\partial^2 \imap_i}{\partial \trv_\pd \partial \theta_i}\end{array}\right]$.  Accounting for our change of variables, we now have an expression for the reference gradient given by
\begin{equation}
\nabla_r \log\tilde{\rd}(\rrv) =  \bigg(\nabla_\trv\log\td(\trv) -\sum_{i=1}^\pd \left(\frac{\partial \imap_i}{\partial \trv_i}\right)^{-1} H_i(\trv)\bigg) \left [ \nabla \imap(\trv) \right ]^{-1} \label{eq:refgrad}.
\end{equation}  
Note that this expression is only valid at $\trv=\imap^{-1}(\rrv)$. 

The lower triangular structure allows us not only to expand the determinant and obtain \eqref{eq:refgrad}, but also to apply the inverse Jacobian $(\nabla T(\trv))^{-1}$ easily through forward substitution.  Furthermore, computing the Jacobian $\nabla \imap(\trv)$  or the second derivatives in $H_i(\trv)$ is trivial when polynomials or other standard basis functions are used to parameterize the map.



==> Paper4Arxiv 2/pics/mcmc/BodPosterior.tex <==

%\iftoggle{enableTikz}{
\begin{tikzpicture}

\begin{axis}[%
width=0.9\textwidth,
height=0.9\textwidth,
xmin=0.4,
xmax=1.3,
ymin=0.08,
ymax=0.28,
xlabel={$\trv_1$},
ylabel={$\trv_2$},
axis on top=true,
]
\addplot graphics[xmin=0.4,ymin=0.08,xmax=1.3,ymax=0.28] {pics/BodPosterior.pdf};
\end{axis}
\end{tikzpicture}%
%}{
%\includegraphics{pics/tikz-external/sisc_main-figure5.pdf}
%}


==> Paper4Arxiv 2/pics/mcmc/GeodesicPaths.tex <==
\begin{axis}[
xscale=0.85,
xmin=-2.5,
xmax=2.5,
ymin=-9,
ymax=1,
xlabel={$\trv_1$},
ylabel={$\trv_2$}
]

\addplot graphics[xmin=-2.5,xmax=2.5,ymin=-12,ymax=1] {pics/mcmc/GeoPathsBanana.pdf};
\end{axis}


==> Paper4Arxiv 2/pics/mcmc/MaplePosterior/MaplePost.tex <==
%\iftoggle{enableTikz}{

\newcommand{\groupPlotWidth}{0.3000\textwidth}
\begin{tikzpicture}[scale=0.5]
\begin{groupplot}[group style={every plot/.style={enlargelimits=true},group size=10 by 10,xlabels at=edge bottom,ylabels at=edge left, xticklabels at=edge bottom,yticklabels at=edge left,vertical sep=1pt,horizontal sep=1pt},height=\groupPlotWidth, width=\groupPlotWidth,ticks=none,enlargelimits=false]

%%%% ROW 1 %%%%
\nextgroupplot[title={\huge$\theta_{1}$}]
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=0.000,ymax=1.451] {pics/mcmc/MaplePosterior/MaplePost11.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 2 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-0.995,ymax=0.997] {pics/mcmc/MaplePosterior/MaplePost21.pdf};
\nextgroupplot[title={\huge$\theta_{2}$}]
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=0.000,ymax=0.920] {pics/mcmc/MaplePosterior/MaplePost22.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 3 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-0.940,ymax=0.996] {pics/mcmc/MaplePosterior/MaplePost31.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-0.940,ymax=0.996] {pics/mcmc/MaplePosterior/MaplePost32.pdf};
\nextgroupplot[title={\huge$\theta_{3}$}]
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=0.000,ymax=1.077] {pics/mcmc/MaplePosterior/MaplePost33.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 4 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-1.089,ymax=1.165] {pics/mcmc/MaplePosterior/MaplePost41.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-1.089,ymax=1.165] {pics/mcmc/MaplePosterior/MaplePost42.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=-1.089,ymax=1.165] {pics/mcmc/MaplePosterior/MaplePost43.pdf};
\nextgroupplot[title={\huge$\theta_{4}$}]
\addplot graphics[xmin=-1.089,ymin=1.165,xmax=0.000,ymax=1.132] {pics/mcmc/MaplePosterior/MaplePost44.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 5 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-1.972,ymax=1.994] {pics/mcmc/MaplePosterior/MaplePost51.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-1.972,ymax=1.994] {pics/mcmc/MaplePosterior/MaplePost52.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=-1.972,ymax=1.994] {pics/mcmc/MaplePosterior/MaplePost53.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.089,ymin=1.165,xmax=-1.972,ymax=1.994] {pics/mcmc/MaplePosterior/MaplePost54.pdf};
\nextgroupplot[title={\huge$\theta_{5}$}]
\addplot graphics[xmin=-1.972,ymin=1.994,xmax=0.000,ymax=0.834] {pics/mcmc/MaplePosterior/MaplePost55.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 6 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-0.585,ymax=0.378] {pics/mcmc/MaplePosterior/MaplePost61.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-0.585,ymax=0.378] {pics/mcmc/MaplePosterior/MaplePost62.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=-0.585,ymax=0.378] {pics/mcmc/MaplePosterior/MaplePost63.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.089,ymin=1.165,xmax=-0.585,ymax=0.378] {pics/mcmc/MaplePosterior/MaplePost64.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.972,ymin=1.994,xmax=-0.585,ymax=0.378] {pics/mcmc/MaplePosterior/MaplePost65.pdf};
\nextgroupplot[title={\huge$\theta_{6}$}]
\addplot graphics[xmin=-0.585,ymin=0.378,xmax=0.000,ymax=2.168] {pics/mcmc/MaplePosterior/MaplePost66.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 7 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-0.421,ymax=1.011] {pics/mcmc/MaplePosterior/MaplePost71.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-0.421,ymax=1.011] {pics/mcmc/MaplePosterior/MaplePost72.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=-0.421,ymax=1.011] {pics/mcmc/MaplePosterior/MaplePost73.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.089,ymin=1.165,xmax=-0.421,ymax=1.011] {pics/mcmc/MaplePosterior/MaplePost74.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.972,ymin=1.994,xmax=-0.421,ymax=1.011] {pics/mcmc/MaplePosterior/MaplePost75.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.585,ymin=0.378,xmax=-0.421,ymax=1.011] {pics/mcmc/MaplePosterior/MaplePost76.pdf};
\nextgroupplot[title={\huge$\theta_{7}$}]
\addplot graphics[xmin=-0.421,ymin=1.011,xmax=0.000,ymax=1.730] {pics/mcmc/MaplePosterior/MaplePost77.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 8 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-2.078,ymax=1.456] {pics/mcmc/MaplePosterior/MaplePost81.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-2.078,ymax=1.456] {pics/mcmc/MaplePosterior/MaplePost82.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=-2.078,ymax=1.456] {pics/mcmc/MaplePosterior/MaplePost83.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.089,ymin=1.165,xmax=-2.078,ymax=1.456] {pics/mcmc/MaplePosterior/MaplePost84.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.972,ymin=1.994,xmax=-2.078,ymax=1.456] {pics/mcmc/MaplePosterior/MaplePost85.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.585,ymin=0.378,xmax=-2.078,ymax=1.456] {pics/mcmc/MaplePosterior/MaplePost86.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.421,ymin=1.011,xmax=-2.078,ymax=1.456] {pics/mcmc/MaplePosterior/MaplePost87.pdf};
\nextgroupplot[title={\huge$\theta_{8}$}]
\addplot graphics[xmin=-2.078,ymin=1.456,xmax=0.000,ymax=0.920] {pics/mcmc/MaplePosterior/MaplePost88.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 9 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost91.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost92.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost93.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.089,ymin=1.165,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost94.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.972,ymin=1.994,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost95.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.585,ymin=0.378,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost96.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.421,ymin=1.011,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost97.pdf};
\nextgroupplot
\addplot graphics[xmin=-2.078,ymin=1.456,xmax=-2.830,ymax=2.885] {pics/mcmc/MaplePosterior/MaplePost98.pdf};
\nextgroupplot[title={\huge$\theta_{9}$}]
\addplot graphics[xmin=-2.830,ymin=2.885,xmax=0.000,ymax=0.579] {pics/mcmc/MaplePosterior/MaplePost99.pdf};

\nextgroupplot[group/empty plot]

%%%% ROW 10 %%%%
\nextgroupplot
\addplot graphics[xmin=-0.825,ymin=0.584,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost101.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.995,ymin=0.997,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost102.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.940,ymin=0.996,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost103.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.089,ymin=1.165,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost104.pdf};
\nextgroupplot
\addplot graphics[xmin=-1.972,ymin=1.994,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost105.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.585,ymin=0.378,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost106.pdf};
\nextgroupplot
\addplot graphics[xmin=-0.421,ymin=1.011,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost107.pdf};
\nextgroupplot
\addplot graphics[xmin=-2.078,ymin=1.456,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost108.pdf};
\nextgroupplot
\addplot graphics[xmin=-2.830,ymin=2.885,xmax=-3.191,ymax=2.990] {pics/mcmc/MaplePosterior/MaplePost109.pdf};
\nextgroupplot[title={\huge$\theta_{10}$}]
\addplot graphics[xmin=-3.191,ymin=2.990,xmax=0.000,ymax=0.543] {pics/mcmc/MaplePosterior/MaplePost1010.pdf};


\end{groupplot}
\end{tikzpicture}

%}{
%\includegraphics{pics/tikz-external/sisc_main-figure8.pdf}
%}


==> Paper4Arxiv 2/pics/mcmc/MaplePosterior/MapleScatter17.tex <==
%\iftoggle{enableTikz}{

\begin{tikzpicture}
\begin{axis}[width=\textwidth, height=\textwidth, xmin=-1, xmax=0.600000, ymin=-0.650000, ymax=2.5, xlabel={$\trv_1$}, ylabel={$\trv_7$}, axis on top=true]
\addplot graphics[xmin=-1,ymin=-0.65,xmax=0.600000,ymax=2.5] {pics/MapleScatter17.pdf};
\end{axis}
\end{tikzpicture}

%}{
%\includegraphics{pics/tikz-external/sisc_main-figure9.pdf}
%}


==> Paper4Arxiv 2/pics/mcmc/MaplePosterior/MapleScatter36.tex <==
%\iftoggle{enableTikz}{

\begin{tikzpicture}
\begin{axis}[width=\textwidth, height=\textwidth, xmin=-1.00000, xmax=1.000000, ymin=-0.600000, ymax=0.400000, xlabel={$\trv_3$}, ylabel={$\trv_6$}, axis on top=true]
\addplot graphics[xmin=-1,ymin=-0.600000,xmax=1.000000,ymax=0.400000] {pics/MapleScatter36.pdf};
\end{axis}
\end{tikzpicture}

%}{
%\includegraphics{pics/tikz-external/sisc_main-figure10.pdf}
%}


==> Paper4Arxiv 2/pics/mcmc/predPreyPosterior/ppPost.tex <==
%\iftoggle{enableTikz}{

\newcommand{\groupPlotWidth}{0.2000\textwidth}
\begin{tikzpicture}[scale=0.6]
\begin{groupplot}[group style={every plot/.style={enlargelimits=true},group size=8 by 8,xlabels at=edge bottom,ylabels at=edge left, xticklabels at=edge bottom,yticklabels at=edge left,vertical sep=1pt,horizontal sep=1pt},height=\groupPlotWidth,width=\groupPlotWidth,ticks=none,enlargelimits=false]

%%%% ROW 1 %%%%
\nextgroupplot[title={\large$P(0)$}]
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.000,ymax=6.133] {pics/mcmc/predPreyPosterior/ppPost11.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 2 %%%%
\nextgroupplot
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.203,ymax=2.628] {pics/mcmc/predPreyPosterior/ppPost21.pdf};
\nextgroupplot[title={\large$Q(0)$}]
\addplot graphics[xmin=0.203,ymin=2.628,xmax=0.000,ymax=1.226] {pics/mcmc/predPreyPosterior/ppPost22.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 3 %%%%
\nextgroupplot
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.269,ymax=1.583] {pics/mcmc/predPreyPosterior/ppPost31.pdf};
\nextgroupplot
\addplot graphics[xmin=0.203,ymin=2.628,xmax=0.269,ymax=1.583] {pics/mcmc/predPreyPosterior/ppPost32.pdf};
\nextgroupplot[title={\large$r$}]
\addplot graphics[xmin=0.269,ymin=1.583,xmax=0.000,ymax=2.212] {pics/mcmc/predPreyPosterior/ppPost33.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 4 %%%%
\nextgroupplot
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.895,ymax=3.660] {pics/mcmc/predPreyPosterior/ppPost41.pdf};
\nextgroupplot
\addplot graphics[xmin=0.203,ymin=2.628,xmax=0.895,ymax=3.660] {pics/mcmc/predPreyPosterior/ppPost42.pdf};
\nextgroupplot
\addplot graphics[xmin=0.269,ymin=1.583,xmax=0.895,ymax=3.660] {pics/mcmc/predPreyPosterior/ppPost43.pdf};
\nextgroupplot[title={\large$K$}]
\addplot graphics[xmin=0.895,ymin=3.660,xmax=0.000,ymax=1.288] {pics/mcmc/predPreyPosterior/ppPost44.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 5 %%%%
\nextgroupplot
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.605,ymax=5.573] {pics/mcmc/predPreyPosterior/ppPost51.pdf};
\nextgroupplot
\addplot graphics[xmin=0.203,ymin=2.628,xmax=0.605,ymax=5.573] {pics/mcmc/predPreyPosterior/ppPost52.pdf};
\nextgroupplot
\addplot graphics[xmin=0.269,ymin=1.583,xmax=0.605,ymax=5.573] {pics/mcmc/predPreyPosterior/ppPost53.pdf};
\nextgroupplot
\addplot graphics[xmin=0.895,ymin=3.660,xmax=0.605,ymax=5.573] {pics/mcmc/predPreyPosterior/ppPost54.pdf};
\nextgroupplot[title={\large$s$}]
\addplot graphics[xmin=0.605,ymin=5.573,xmax=0.000,ymax=0.507] {pics/mcmc/predPreyPosterior/ppPost55.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 6 %%%%
\nextgroupplot
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.566,ymax=9.850] {pics/mcmc/predPreyPosterior/ppPost61.pdf};
\nextgroupplot
\addplot graphics[xmin=0.203,ymin=2.628,xmax=0.566,ymax=9.850] {pics/mcmc/predPreyPosterior/ppPost62.pdf};
\nextgroupplot
\addplot graphics[xmin=0.269,ymin=1.583,xmax=0.566,ymax=9.850] {pics/mcmc/predPreyPosterior/ppPost63.pdf};
\nextgroupplot
\addplot graphics[xmin=0.895,ymin=3.660,xmax=0.566,ymax=9.850] {pics/mcmc/predPreyPosterior/ppPost64.pdf};
\nextgroupplot
\addplot graphics[xmin=0.605,ymin=5.573,xmax=0.566,ymax=9.850] {pics/mcmc/predPreyPosterior/ppPost65.pdf};
\nextgroupplot[title={\large$a$}]
\addplot graphics[xmin=0.566,ymin=9.850,xmax=0.000,ymax=0.304] {pics/mcmc/predPreyPosterior/ppPost66.pdf};

\nextgroupplot[group/empty plot]
\nextgroupplot[group/empty plot]

%%%% ROW 7 %%%%
\nextgroupplot
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.134,ymax=2.544] {pics/mcmc/predPreyPosterior/ppPost71.pdf};
\nextgroupplot
\addplot graphics[xmin=0.203,ymin=2.628,xmax=0.134,ymax=2.544] {pics/mcmc/predPreyPosterior/ppPost72.pdf};
\nextgroupplot
\addplot graphics[xmin=0.269,ymin=1.583,xmax=0.134,ymax=2.544] {pics/mcmc/predPreyPosterior/ppPost73.pdf};
\nextgroupplot
\addplot graphics[xmin=0.895,ymin=3.660,xmax=0.134,ymax=2.544] {pics/mcmc/predPreyPosterior/ppPost74.pdf};
\nextgroupplot
\addplot graphics[xmin=0.605,ymin=5.573,xmax=0.134,ymax=2.544] {pics/mcmc/predPreyPosterior/ppPost75.pdf};
\nextgroupplot
\addplot graphics[xmin=0.566,ymin=9.850,xmax=0.134,ymax=2.544] {pics/mcmc/predPreyPosterior/ppPost76.pdf};
\nextgroupplot[title={\large$u$}]
\addplot graphics[xmin=0.134,ymin=2.544,xmax=0.000,ymax=1.875] {pics/mcmc/predPreyPosterior/ppPost77.pdf};

\nextgroupplot[group/empty plot]

%%%% ROW 8 %%%%
\nextgroupplot
\addplot graphics[xmin=0.737,ymin=1.255,xmax=0.273,ymax=2.028] {pics/mcmc/predPreyPosterior/ppPost81.pdf};
\nextgroupplot
\addplot graphics[xmin=0.203,ymin=2.628,xmax=0.273,ymax=2.028] {pics/mcmc/predPreyPosterior/ppPost82.pdf};
\nextgroupplot
\addplot graphics[xmin=0.269,ymin=1.583,xmax=0.273,ymax=2.028] {pics/mcmc/predPreyPosterior/ppPost83.pdf};
\nextgroupplot
\addplot graphics[xmin=0.895,ymin=3.660,xmax=0.273,ymax=2.028] {pics/mcmc/predPreyPosterior/ppPost84.pdf};
\nextgroupplot
\addplot graphics[xmin=0.605,ymin=5.573,xmax=0.273,ymax=2.028] {pics/mcmc/predPreyPosterior/ppPost85.pdf};
\nextgroupplot
\addplot graphics[xmin=0.566,ymin=9.850,xmax=0.273,ymax=2.028] {pics/mcmc/predPreyPosterior/ppPost86.pdf};
\nextgroupplot
\addplot graphics[xmin=0.134,ymin=2.544,xmax=0.273,ymax=2.028] {pics/mcmc/predPreyPosterior/ppPost87.pdf};
\nextgroupplot[title={\large$v$}]
\addplot graphics[xmin=0.273,ymin=2.028,xmax=0.000,ymax=2.486] {pics/mcmc/predPreyPosterior/ppPost88.pdf};


\end{groupplot}
\end{tikzpicture}

%}{
%\includegraphics{pics/tikz-external/sisc_main-figure7.pdf}
%}



==> pics/mcmc/GeodesicPaths.tex <==
\begin{axis}[
xscale=0.85,
xmin=-2.5,
xmax=2.5,
ymin=-9,
ymax=1,
xlabel={$\trv_1$},
ylabel={$\trv_2$}
]

\addplot graphics[xmin=-2.5,xmax=2.5,ymin=-12,ymax=1] {pics/mcmc/GeoPathsBanana.pdf};
\end{axis}

